Chaos Gaussian Splatting: Polynomial Regression with Gaussian Splats for Chaotic Maps with Gradient Discontinuities

Polynomial regression forecasts noise-free, fully observed, low-dimensional chaotic systems almost to machine precision, but many one-step maps are not low-degree polynomials: maps with kinks, and flows observed through a single coordinate. We introduce chaos Gaussian splatting (CGS), which models the map as a polynomial trend plus Gaussian "splats", local quadratics split and pruned as in Gaussian splatting and fitted in closed form, reducing to polynomial regression where that suffices. Compact mode fits one splat field; full mode, for kinked maps, gives the splats hinges, combines six splat fields and defers, where they disagree, to a referee that locates kinks in the training data. In a pre-registered test on fresh initial conditions of ten systems (38 units), full mode had a lower one-step error than the S-map and the Farmer--Sidorowich predictor, each given every input view CGS uses, on every unit, with a median error 72 times lower; it predicts 24 times more slowly. In closed loop (post hoc) its forecasts outlasted those methods' and an echo state network's on every map unit, by 1 to 7 steps. On six scalar kinked maps with $10^5$ points, compact mode met an accuracy target set by the Farmer--Sidorowich predictor in 67 of 89 runs and then used 25--76 times less memory than any local model meeting it. Once observation noise dominates, the methods' errors agree within a factor of 1.5 (35 of 36 cases, a second pre-registered study); on a measured laser series CGS was not more accurate than the S-map.

==> tables/budget_numbers.tex <==
% generated by paper/budget_numbers.py from results/budget -- do not edit
\makeatletter
\@namedef{num@bud.abl.max}{4.9\times10^{5}}
\@namedef{num@bud.abl.min}{6.8}
\@namedef{num@bud.abl.series3}{1}
\@namedef{num@bud.bcnf.1000.gm}{0.5}
\@namedef{num@bud.bcnf.1000.gm.hi}{1.2}
\@namedef{num@bud.bcnf.1000.gm.lo}{0.02}
\@namedef{num@bud.bcnf.1000.gt}{8}
\@namedef{num@bud.bcnf.1000.q}{7.1\times10^{6}}
\@namedef{num@bud.bcnf.1000.runs}{15}
\@namedef{num@bud.bcnf.1000.test}{4}
\@namedef{num@bud.bcnf.1000.val}{6}
\@namedef{num@bud.bcnf.10000.gm}{0.44}
\@namedef{num@bud.bcnf.10000.gm.hi}{1.1}
\@namedef{num@bud.bcnf.10000.gm.lo}{0.3}
\@namedef{num@bud.bcnf.10000.gt}{4.3}
\@namedef{num@bud.bcnf.10000.q}{9.4\times10^{6}}
\@namedef{num@bud.bcnf.10000.runs}{15}
\@namedef{num@bud.bcnf.10000.test}{2}
\@namedef{num@bud.bcnf.10000.val}{6}
\@namedef{num@bud.bcnf.100000.gm}{1.1}
\@namedef{num@bud.bcnf.100000.gm.hi}{1.6}
\@namedef{num@bud.bcnf.100000.gm.lo}{0.62}
\@namedef{num@bud.bcnf.100000.gt}{5.8}
\@namedef{num@bud.bcnf.100000.q}{10^{8}}
\@namedef{num@bud.bcnf.100000.runs}{15}
\@namedef{num@bud.bcnf.100000.test}{5}
\@namedef{num@bud.bcnf.100000.val}{13}
\@namedef{num@bud.bcnf.900000.gm}{2.2}
\@namedef{num@bud.bcnf.900000.gm.hi}{4}
\@namedef{num@bud.bcnf.900000.gm.lo}{1.2}
\@namedef{num@bud.bcnf.900000.gt}{6}
\@namedef{num@bud.bcnf.900000.q}{3.6\times10^{8}}
\@namedef{num@bud.bcnf.900000.runs}{15}
\@namedef{num@bud.bcnf.900000.test}{9}
\@namedef{num@bud.bcnf.900000.val}{14}
\@namedef{num@bud.bentlogistic.1000.gm}{1.3}
\@namedef{num@bud.bentlogistic.1000.gm.hi}{2}
\@namedef{num@bud.bentlogistic.1000.gm.lo}{0.53}
\@namedef{num@bud.bentlogistic.1000.gt}{5}
\@namedef{num@bud.bentlogistic.1000.q}{9.3\times10^{6}}
\@namedef{num@bud.bentlogistic.1000.runs}{15}
\@namedef{num@bud.bentlogistic.1000.test}{4}
\@namedef{num@bud.bentlogistic.1000.val}{15}
\@namedef{num@bud.bentlogistic.10000.gm}{2.3}
\@namedef{num@bud.bentlogistic.10000.gm.hi}{4.1}
\@namedef{num@bud.bentlogistic.10000.gm.lo}{1.1}
\@namedef{num@bud.bentlogistic.10000.gt}{5.1}
\@namedef{num@bud.bentlogistic.10000.q}{2.0\times10^{7}}
\@namedef{num@bud.bentlogistic.10000.runs}{15}
\@namedef{num@bud.bentlogistic.10000.test}{6}
\@namedef{num@bud.bentlogistic.10000.val}{12}
\@namedef{num@bud.bentlogistic.100000.gm}{25}
\@namedef{num@bud.bentlogistic.100000.gm.hi}{102}
\@namedef{num@bud.bentlogistic.100000.gm.lo}{14}
\@namedef{num@bud.bentlogistic.100000.gt}{11}
\@namedef{num@bud.bentlogistic.100000.q}{5.1\times10^{7}}
\@namedef{num@bud.bentlogistic.100000.runs}{14}
\@namedef{num@bud.bentlogistic.100000.test}{10}
\@namedef{num@bud.bentlogistic.100000.val}{13}
\@namedef{num@bud.bentlogistic.900000.gm}{104}
\@namedef{num@bud.bentlogistic.900000.gm.hi}{114}
\@namedef{num@bud.bentlogistic.900000.gm.lo}{98}
\@namedef{num@bud.bentlogistic.900000.gt}{14}
\@namedef{num@bud.bentlogistic.900000.q}{2.5\times10^{8}}
\@namedef{num@bud.bentlogistic.900000.runs}{15}
\@namedef{num@bud.bentlogistic.900000.test}{10}
\@namedef{num@bud.bentlogistic.900000.val}{13}
\@namedef{num@bud.crash}{curvedtent, $n=10^3$, initial condition 3, seed 2}
\@namedef{num@bud.curvedtent.1000.gm}{0.69}
\@namedef{num@bud.curvedtent.1000.gm.hi}{1.5}
\@namedef{num@bud.curvedtent.1000.gm.lo}{0.6}
\@namedef{num@bud.curvedtent.1000.gt}{4.6}
\@namedef{num@bud.curvedtent.1000.q}{9.8\times10^{6}}
\@namedef{num@bud.curvedtent.1000.runs}{14}
\@namedef{num@bud.curvedtent.1000.test}{8}
\@namedef{num@bud.curvedtent.1000.val}{13}
\@namedef{num@bud.curvedtent.10000.gm}{8.2}
\@namedef{num@bud.curvedtent.10000.gm.hi}{16}
\@namedef{num@bud.curvedtent.10000.gm.lo}{3.7}
\@namedef{num@bud.curvedtent.10000.gt}{4.8}
\@namedef{num@bud.curvedtent.10000.q}{2.3\times10^{7}}
\@namedef{num@bud.curvedtent.10000.runs}{15}
\@namedef{num@bud.curvedtent.10000.test}{3}
\@namedef{num@bud.curvedtent.10000.val}{7}
\@namedef{num@bud.curvedtent.100000.gm}{49}
\@namedef{num@bud.curvedtent.100000.gm.hi}{110}
\@namedef{num@bud.curvedtent.100000.gm.lo}{18}
\@namedef{num@bud.curvedtent.100000.gt}{4.4}
\@namedef{num@bud.curvedtent.100000.q}{1.7\times10^{8}}
\@namedef{num@bud.curvedtent.100000.runs}{15}
\@namedef{num@bud.curvedtent.100000.test}{5}
\@namedef{num@bud.curvedtent.100000.val}{12}
\@namedef{num@bud.curvedtent.900000.gm}{223}
\@namedef{num@bud.curvedtent.900000.gm.hi}{303}
\@namedef{num@bud.curvedtent.900000.gm.lo}{85}
\@namedef{num@bud.curvedtent.900000.gt}{5.3}
\@namedef{num@bud.curvedtent.900000.q}{5.0\times10^{8}}
\@namedef{num@bud.curvedtent.900000.runs}{15}
\@namedef{num@bud.curvedtent.900000.test}{15}
\@namedef{num@bud.curvedtent.900000.val}{15}
\@namedef{num@bud.k1.100000.gm.max}{76}
\@namedef{num@bud.k1.100000.gm.min}{25}
\@namedef{num@bud.k1.100000.gmrt.max}{214}
\@namedef{num@bud.k1.100000.gmrt.min}{77}
\@namedef{num@bud.k1.100000.gsingle.max}{1.7}
\@namedef{num@bud.k1.100000.gsingle.min}{1}
\@namedef{num@bud.k1.100000.gt.max}{11}
\@namedef{num@bud.k1.100000.gt.min}{4.2}
\@namedef{num@bud.k1.100000.gtraj.max}{1.6}
\@namedef{num@bud.k1.100000.gtraj.min}{1}
\@namedef{num@bud.k1.100000.loadcs.max}{1.3}
\@namedef{num@bud.k1.100000.loadloc.max}{18}
\@namedef{num@bud.k1.100000.loadloc.min}{2.9}
\@namedef{num@bud.k1.100000.q.max}{1.7\times10^{8}}
\@namedef{num@bud.k1.100000.q.min}{5.1\times10^{7}}
\@namedef{num@bud.k1.100000.qt.max}{11}
\@namedef{num@bud.k1.100000.qt.min}{9}
\@namedef{num@bud.k1.100000.runs}{89}
\@namedef{num@bud.k1.100000.single.max}{0.3}
\@namedef{num@bud.k1.100000.single.min}{0.2}
\@namedef{num@bud.k1.100000.test}{42}
\@namedef{num@bud.k1.100000.val}{67}
\@namedef{num@bud.k1.900000.gm.max}{268}
\@namedef{num@bud.k1.900000.gm.min}{57}
\@namedef{num@bud.k1.900000.gmrt.max}{1012}
\@namedef{num@bud.k1.900000.gmrt.min}{178}
\@namedef{num@bud.k1.900000.gsingle.max}{1.8}
\@namedef{num@bud.k1.900000.gsingle.min}{1.2}
\@namedef{num@bud.k1.900000.gt.max}{14}
\@namedef{num@bud.k1.900000.gt.min}{5.3}
\@namedef{num@bud.k1.900000.gtraj.max}{1.8}
\@namedef{num@bud.k1.900000.gtraj.min}{1.2}
\@namedef{num@bud.k1.900000.loadcs.max}{2}
\@namedef{num@bud.k1.900000.loadloc.max}{424}
\@namedef{num@bud.k1.900000.loadloc.min}{26}
\@namedef{num@bud.k1.900000.q.max}{6.6\times10^{8}}
\@namedef{num@bud.k1.900000.q.min}{2.5\times10^{8}}
\@namedef{num@bud.k1.900000.qt.max}{1.7}
\@namedef{num@bud.k1.900000.qt.min}{1}
\@namedef{num@bud.k1.900000.runs}{90}
\@namedef{num@bud.k1.900000.single.max}{0.3}
\@namedef{num@bud.k1.900000.single.min}{0.2}
\@namedef{num@bud.k1.900000.test}{68}
\@namedef{num@bud.k1.900000.val}{73}
\@namedef{num@bud.lozi.1000.gm}{0.27}
\@namedef{num@bud.lozi.1000.gm.hi}{0.32}
\@namedef{num@bud.lozi.1000.gm.lo}{0.13}
\@namedef{num@bud.lozi.1000.gt}{6.8}
\@namedef{num@bud.lozi.1000.q}{5.7\times10^{6}}
\@namedef{num@bud.lozi.1000.runs}{15}
\@namedef{num@bud.lozi.1000.test}{7}
\@namedef{num@bud.lozi.1000.val}{11}
\@namedef{num@bud.lozi.10000.gm}{0.53}
\@namedef{num@bud.lozi.10000.gm.hi}{0.6}
\@namedef{num@bud.lozi.10000.gm.lo}{0.3}
\@namedef{num@bud.lozi.10000.gt}{3.8}
\@namedef{num@bud.lozi.10000.q}{1.3\times10^{7}}
\@namedef{num@bud.lozi.10000.runs}{15}
\@namedef{num@bud.lozi.10000.test}{3}
\@namedef{num@bud.lozi.10000.val}{8}
\@namedef{num@bud.lozi.100000.runs}{14}
\@namedef{num@bud.lozi.100000.test}{0}
\@namedef{num@bud.lozi.100000.val}{0}
\@namedef{num@bud.lozi.900000.gm}{8.4}
\@namedef{num@bud.lozi.900000.gm.hi}{35}
\@namedef{num@bud.lozi.900000.gm.lo}{1.2}
\@namedef{num@bud.lozi.900000.gt}{7.5}
\@namedef{num@bud.lozi.900000.q}{5.6\times10^{8}}
\@namedef{num@bud.lozi.900000.runs}{15}
\@namedef{num@bud.lozi.900000.test}{1}
\@namedef{num@bud.lozi.900000.val}{7}
\@namedef{num@bud.quadtent.1000.gm}{0.62}
\@namedef{num@bud.quadtent.1000.gm.hi}{1.1}
\@namedef{num@bud.quadtent.1000.gm.lo}{0.34}
\@namedef{num@bud.quadtent.1000.gt}{4.6}
\@namedef{num@bud.quadtent.1000.q}{8.1\times10^{6}}
\@namedef{num@bud.quadtent.1000.runs}{15}
\@namedef{num@bud.quadtent.1000.test}{13}
\@namedef{num@bud.quadtent.1000.val}{15}
\@namedef{num@bud.quadtent.10000.gm}{14}
\@namedef{num@bud.quadtent.10000.gm.hi}{18}
\@namedef{num@bud.quadtent.10000.gm.lo}{6.1}
\@namedef{num@bud.quadtent.10000.gt}{5}
\@namedef{num@bud.quadtent.10000.q}{1.8\times10^{7}}
\@namedef{num@bud.quadtent.10000.runs}{15}
\@namedef{num@bud.quadtent.10000.test}{5}
\@namedef{num@bud.quadtent.10000.val}{8}
\@namedef{num@bud.quadtent.100000.gm}{76}
\@namedef{num@bud.quadtent.100000.gm.hi}{130}
\@namedef{num@bud.quadtent.100000.gm.lo}{39}
\@namedef{num@bud.quadtent.100000.gt}{4.2}
\@namedef{num@bud.quadtent.100000.q}{9.7\times10^{7}}
\@namedef{num@bud.quadtent.100000.runs}{15}
\@namedef{num@bud.quadtent.100000.test}{2}
\@namedef{num@bud.quadtent.100000.val}{3}
\@namedef{num@bud.quadtent.900000.gm}{68}
\@namedef{num@bud.quadtent.900000.gm.hi}{158}
\@namedef{num@bud.quadtent.900000.gm.lo}{49}
\@namedef{num@bud.quadtent.900000.gt}{9.2}
\@namedef{num@bud.quadtent.900000.q}{4.5\times10^{8}}
\@namedef{num@bud.quadtent.900000.runs}{15}
\@namedef{num@bud.quadtent.900000.test}{5}
\@namedef{num@bud.quadtent.900000.val}{6}
\@namedef{num@bud.rossler.1000.gm}{0.57}
\@namedef{num@bud.rossler.1000.gm.hi}{1.1}
\@namedef{num@bud.rossler.1000.gm.lo}{0.12}
\@namedef{num@bud.rossler.1000.gt}{118}
\@namedef{num@bud.rossler.1000.q}{2.2\times10^{6}}
\@namedef{num@bud.rossler.1000.runs}{15}
\@namedef{num@bud.rossler.1000.test}{1}
\@namedef{num@bud.rossler.1000.val}{3}
\@namedef{num@bud.rossler.10000.runs}{11}
\@namedef{num@bud.rossler.10000.test}{0}
\@namedef{num@bud.rossler.10000.val}{0}
\@namedef{num@bud.rossler.100000.runs}{1}
\@namedef{num@bud.rossler.100000.test}{0}
\@namedef{num@bud.rossler.100000.val}{0}
\@namedef{num@bud.rt.cloud.fmax}{1.4\times10^{3}}
\@namedef{num@bud.rt.cloud.fmed}{2}
\@namedef{num@bud.rt.cloud.full}{2}
\@namedef{num@bud.rt.cloud.ghz}{2.80}
\@namedef{num@bud.rt.cloud.levels}{7}
\@namedef{num@bud.rt.cloud.local}{1157}
\@namedef{num@bud.rt.cloud.localrel}{5.1\times10^{-5}}
\@namedef{num@bud.rt.cloud.nlevels}{198}
\@namedef{num@bud.rt.cloud.nlocal}{1157}
\@namedef{num@bud.rt.cloud.notfull}{17}
\@namedef{num@bud.rt.cloud.ntargets}{684}
\@namedef{num@bud.rt.cloud.numpy}{1.26.4}
\@namedef{num@bud.rt.cloud.runs}{19}
\@namedef{num@bud.rt.cloud.targets}{659}
\@namedef{num@bud.rt.colab.fmax}{1.25}
\@namedef{num@bud.rt.colab.fmed}{1}
\@namedef{num@bud.rt.colab.full}{18}
\@namedef{num@bud.rt.colab.ghz}{2.00}
\@namedef{num@bud.rt.colab.levels}{190}
\@namedef{num@bud.rt.colab.local}{1157}
\@namedef{num@bud.rt.colab.localrel}{5.1\times10^{-5}}
\@namedef{num@bud.rt.colab.nlevels}{196}
\@namedef{num@bud.rt.colab.nlocal}{1157}
\@namedef{num@bud.rt.colab.notfull}{1}
\@namedef{num@bud.rt.colab.ntargets}{684}
\@namedef{num@bud.rt.colab.numpy}{2.1.3}
\@namedef{num@bud.rt.colab.runs}{19}
\@namedef{num@bud.rt.colab.targets}{684}
\@namedef{num@bud.rt.seed.fmax}{8.6\times10^{3}}
\@namedef{num@bud.rt.seed.fmed}{2.5}
\@namedef{num@bud.runs.A}{480}
\@namedef{num@bud.runs.A.done}{469}
\@namedef{num@bud.runs.done}{554}
\@namedef{num@bud.runs.planned}{565}
\@namedef{num@bud.runs.timed}{531}
\@namedef{num@bud.second.maxrel}{$3.4\times10^{-7}$}
\@namedef{num@bud.second.models}{143}
\@namedef{num@bud.second.same}{51}
\@namedef{num@bud.series3.1000.gm}{2}
\@namedef{num@bud.series3.1000.gm.hi}{2.9}
\@namedef{num@bud.series3.1000.gm.lo}{1}
\@namedef{num@bud.series3.1000.gt}{19}
\@namedef{num@bud.series3.1000.q}{10^{6}}
\@namedef{num@bud.series3.1000.runs}{15}
\@namedef{num@bud.series3.1000.test}{10}
\@namedef{num@bud.series3.1000.val}{12}
\@namedef{num@bud.series3.10000.gm}{9.8}
\@namedef{num@bud.series3.10000.gm.hi}{18}
\@namedef{num@bud.series3.10000.gm.lo}{8.2}
\@namedef{num@bud.series3.10000.gt}{86}
\@namedef{num@bud.series3.10000.q}{1.6\times10^{5}}
\@namedef{num@bud.series3.10000.runs}{15}
\@namedef{num@bud.series3.10000.test}{15}
\@namedef{num@bud.series3.10000.val}{15}
\@namedef{num@bud.series3.100000.gm}{40}
\@namedef{num@bud.series3.100000.gm.hi}{49}
\@namedef{num@bud.series3.100000.gm.lo}{27}
\@namedef{num@bud.series3.100000.gt}{160}
\@namedef{num@bud.series3.100000.q}{10^{5}}
\@namedef{num@bud.series3.100000.runs}{15}
\@namedef{num@bud.series3.100000.test}{15}
\@namedef{num@bud.series3.100000.val}{15}
\@namedef{num@bud.series3.900000.gm}{88}
\@namedef{num@bud.series3.900000.gm.hi}{107}
\@namedef{num@bud.series3.900000.gm.lo}{5.4}
\@namedef{num@bud.series3.900000.gt}{384}
\@namedef{num@bud.series3.900000.runs}{5}
\@namedef{num@bud.series3.900000.test}{5}
\@namedef{num@bud.series3.900000.val}{5}
\@namedef{num@bud.series4.1000.gm}{0.54}
\@namedef{num@bud.series4.1000.gm.hi}{0.9}
\@namedef{num@bud.series4.1000.gm.lo}{0.26}
\@namedef{num@bud.series4.1000.gt}{4.4}
\@namedef{num@bud.series4.1000.q}{1.2\times10^{7}}
\@namedef{num@bud.series4.1000.runs}{15}
\@namedef{num@bud.series4.1000.test}{8}
\@namedef{num@bud.series4.1000.val}{14}
\@namedef{num@bud.series4.10000.gm}{4.1}
\@namedef{num@bud.series4.10000.gm.hi}{12}
\@namedef{num@bud.series4.10000.gm.lo}{2.3}
\@namedef{num@bud.series4.10000.gt}{4.2}
\@namedef{num@bud.series4.10000.q}{3.8\times10^{7}}
\@namedef{num@bud.series4.10000.runs}{15}
\@namedef{num@bud.series4.10000.test}{2}
\@namedef{num@bud.series4.10000.val}{3}
\@namedef{num@bud.series4.100000.gm}{39}
\@namedef{num@bud.series4.100000.gm.hi}{71}
\@namedef{num@bud.series4.100000.gm.lo}{13}
\@namedef{num@bud.series4.100000.gt}{7.4}
\@namedef{num@bud.series4.100000.q}{9.0\times10^{7}}
\@namedef{num@bud.series4.100000.runs}{15}
\@namedef{num@bud.series4.100000.test}{7}
\@namedef{num@bud.series4.100000.val}{15}
\@namedef{num@bud.series4.900000.gm}{57}
\@namedef{num@bud.series4.900000.gm.hi}{89}
\@namedef{num@bud.series4.900000.gm.lo}{16}
\@namedef{num@bud.series4.900000.gt}{10}
\@namedef{num@bud.series4.900000.q}{2.8\times10^{8}}
\@namedef{num@bud.series4.900000.runs}{15}
\@namedef{num@bud.series4.900000.test}{12}
\@namedef{num@bud.series4.900000.val}{12}
\@namedef{num@bud.series5.1000.gm}{0.81}
\@namedef{num@bud.series5.1000.gm.hi}{2}
\@namedef{num@bud.series5.1000.gm.lo}{0.3}
\@namedef{num@bud.series5.1000.gt}{4.4}
\@namedef{num@bud.series5.1000.q}{1.1\times10^{7}}
\@namedef{num@bud.series5.1000.runs}{15}
\@namedef{num@bud.series5.1000.test}{3}
\@namedef{num@bud.series5.1000.val}{14}
\@namedef{num@bud.series5.10000.gm}{3.7}
\@namedef{num@bud.series5.10000.gm.hi}{14}
\@namedef{num@bud.series5.10000.gm.lo}{1.7}
\@namedef{num@bud.series5.10000.gt}{5.6}
\@namedef{num@bud.series5.10000.q}{2.0\times10^{7}}
\@namedef{num@bud.series5.10000.runs}{15}
\@namedef{num@bud.series5.10000.test}{5}
\@namedef{num@bud.series5.10000.val}{8}
\@namedef{num@bud.series5.100000.gm}{27}
\@namedef{num@bud.series5.100000.gm.hi}{36}
\@namedef{num@bud.series5.100000.gm.lo}{17}
\@namedef{num@bud.series5.100000.gt}{6.7}
\@namedef{num@bud.series5.100000.q}{8.8\times10^{7}}
\@namedef{num@bud.series5.100000.runs}{15}
\@namedef{num@bud.series5.100000.test}{12}
\@namedef{num@bud.series5.100000.val}{13}
\@namedef{num@bud.series5.900000.gm}{72}
\@namedef{num@bud.series5.900000.gm.hi}{249}
\@namedef{num@bud.series5.900000.gm.lo}{20}
\@namedef{num@bud.series5.900000.gt}{6.3}
\@namedef{num@bud.series5.900000.q}{6.6\times10^{8}}
\@namedef{num@bud.series5.900000.runs}{15}
\@namedef{num@bud.series5.900000.test}{14}
\@namedef{num@bud.series5.900000.val}{15}
\@namedef{num@bud.series6.1000.gm}{1.2}
\@namedef{num@bud.series6.1000.gm.hi}{1.4}
\@namedef{num@bud.series6.1000.gm.lo}{0.55}
\@namedef{num@bud.series6.1000.gt}{4.5}
\@namedef{num@bud.series6.1000.q}{1.2\times10^{7}}
\@namedef{num@bud.series6.1000.runs}{15}
\@namedef{num@bud.series6.1000.test}{10}
\@namedef{num@bud.series6.1000.val}{15}
\@namedef{num@bud.series6.10000.gm}{3.8}
\@namedef{num@bud.series6.10000.gm.hi}{15}
\@namedef{num@bud.series6.10000.gm.lo}{1.2}
\@namedef{num@bud.series6.10000.gt}{4.9}
\@namedef{num@bud.series6.10000.q}{2.2\times10^{7}}
\@namedef{num@bud.series6.10000.runs}{15}
\@namedef{num@bud.series6.10000.test}{8}
\@namedef{num@bud.series6.10000.val}{10}
\@namedef{num@bud.series6.100000.gm}{41}
\@namedef{num@bud.series6.100000.gm.hi}{123}
\@namedef{num@bud.series6.100000.gm.lo}{10}
\@namedef{num@bud.series6.100000.gt}{4.9}
\@namedef{num@bud.series6.100000.q}{1.7\times10^{8}}
\@namedef{num@bud.series6.100000.runs}{15}
\@namedef{num@bud.series6.100000.test}{6}
\@namedef{num@bud.series6.100000.val}{11}
\@namedef{num@bud.series6.900000.gm}{268}
\@namedef{num@bud.series6.900000.gm.hi}{920}
\@namedef{num@bud.series6.900000.gm.lo}{204}
\@namedef{num@bud.series6.900000.gt}{7.9}
\@namedef{num@bud.series6.900000.q}{3.9\times10^{8}}
\@namedef{num@bud.series6.900000.runs}{15}
\@namedef{num@bud.series6.900000.test}{12}
\@namedef{num@bud.series6.900000.val}{12}
\makeatother


==> tables/extra_numbers.tex <==
% generated by make_extra_baselines.py -- do not edit
\makeatletter
\@namedef{num@extra.units}{20}
\@namedef{num@extra.methods}{9}
\@namedef{num@extra.cs.best}{20}
\@namedef{num@extra.cs.best20}{20}
\@namedef{num@extra.ngrc.units}{20}
\@namedef{num@extra.ngrc.cswins}{20}
\@namedef{num@extra.ngrc.locwins}{3}
\@namedef{num@extra.esn.units}{20}
\@namedef{num@extra.esn.cswins}{20}
\@namedef{num@extra.esn.locwins}{2}
\@namedef{num@extra.setar.units}{20}
\@namedef{num@extra.setar.cswins}{20}
\@namedef{num@extra.setar.locwins}{0}
\@namedef{num@extra.gbt.units}{20}
\@namedef{num@extra.gbt.cswins}{20}
\@namedef{num@extra.gbt.locwins}{0}
\@namedef{num@extra.mars.units}{20}
\@namedef{num@extra.mars.cswins}{20}
\@namedef{num@extra.mars.locwins}{4}
\@namedef{num@extra.mlp.units}{20}
\@namedef{num@extra.mlp.cswins}{20}
\@namedef{num@extra.mlp.locwins}{0}
\@namedef{num@extra.krr.units}{20}
\@namedef{num@extra.krr.cswins}{20}
\@namedef{num@extra.krr.locwins}{3}
\@namedef{num@extra.panda.units}{20}
\@namedef{num@extra.panda.cswins}{20}
\@namedef{num@extra.panda.locwins}{0}
\@namedef{num@extra.timegs.units}{20}
\@namedef{num@extra.timegs.cswins}{20}
\@namedef{num@extra.timegs.locwins}{0}
\@namedef{num@extra.panda.min}{8\times10^{-3}}
\@namedef{num@extra.panda.max}{2\times10^{-1}}
\@namedef{num@extra.panda.ratio.min}{10^{9}}
\@namedef{num@extra.panda.ratio.max}{10^{14}}
\@namedef{num@extra.panda.u20maps.min}{0.87}
\@namedef{num@extra.panda.u20maps.max}{1.01}
\@namedef{num@extra.timegs.min}{6\times10^{-4}}
\@namedef{num@extra.timegs.max}{5\times10^{-2}}
\@namedef{num@extra.timegs.ratio.min}{10^{7}}
\@namedef{num@extra.timegs.ratio.max}{10^{13}}
\@namedef{num@extra.timegs.u20maps.min}{0.78}
\@namedef{num@extra.timegs.u20maps.max}{0.99}
\makeatother


==> tables/full_numbers.tex <==
% generated by experiments/overleaf/make_full_mode_tables.py -- do not edit
\makeatletter
\@namedef{num@full.cap.rossler}{25{,}000}
\@namedef{num@full.cap.series1}{20{,}000}
\@namedef{num@full.capr2.rossler.10000}{0.61}
\@namedef{num@full.capr2.rossler.100000}{0.62}
\@namedef{num@full.capr2.series1.1000}{1.00}
\@namedef{num@full.capr2.series1.10000}{1.00}
\@namedef{num@full.capr2.series1.100000}{1.00}
\@namedef{num@full.h.bcnf.1000}{85}
\@namedef{num@full.h.bcnf.10000}{86}
\@namedef{num@full.h.bcnf.100000}{90}
\@namedef{num@full.h.bentlogistic.1000}{47}
\@namedef{num@full.h.bentlogistic.10000}{49}
\@namedef{num@full.h.bentlogistic.100000}{51}
\@namedef{num@full.h.curvedtent.1000}{68}
\@namedef{num@full.h.curvedtent.10000}{68}
\@namedef{num@full.h.curvedtent.100000}{68}
\@namedef{num@full.h.henon.10000}{87}
\@namedef{num@full.h.henon.100000}{89}
\@namedef{num@full.h.lorenz.10000}{1542}
\@namedef{num@full.h.lorenz.100000}{3368}
\@namedef{num@full.h.lozi.1000}{76}
\@namedef{num@full.h.lozi.10000}{75}
\@namedef{num@full.h.lozi.100000}{75}
\@namedef{num@full.h.quadtent.1000}{57}
\@namedef{num@full.h.quadtent.10000}{57}
\@namedef{num@full.h.quadtent.100000}{60}
\@namedef{num@full.h.rossler.10000}{more than 25{,}000 (0.61)}
\@namedef{num@full.h.rossler.100000}{more than 25{,}000 (0.62)}
\@namedef{num@full.h.series1.1000}{more than 20{,}000 (1.00)}
\@namedef{num@full.h.series1.10000}{more than 20{,}000 (1.00)}
\@namedef{num@full.h.series1.100000}{more than 20{,}000 (1.00)}
\@namedef{num@full.h.series2.1000}{76}
\@namedef{num@full.h.series2.10000}{76}
\@namedef{num@full.h.series2.100000}{76}
\@namedef{num@full.h.series3.1000}{50}
\@namedef{num@full.h.series3.10000}{51}
\@namedef{num@full.h.series3.100000}{51}
\@namedef{num@full.h.series4.1000}{39}
\@namedef{num@full.h.series4.10000}{39}
\@namedef{num@full.h.series4.100000}{41}
\@namedef{num@full.h.series5.1000}{32}
\@namedef{num@full.h.series5.10000}{32}
\@namedef{num@full.h.series5.100000}{33}
\@namedef{num@full.h.series6.1000}{26}
\@namedef{num@full.h.series6.10000}{27}
\@namedef{num@full.h.series6.100000}{27}
\@namedef{num@full.h.skewtent.1000}{56}
\@namedef{num@full.h.skewtent.10000}{55}
\@namedef{num@full.h.skewtent.100000}{56}
\@namedef{num@full.ho.mse.gainmax.1000}{2.4\times10^{9}}
\@namedef{num@full.ho.mse.gainmax.10000}{1.9\times10^{7}}
\@namedef{num@full.ho.mse.gainmax.100000}{2.4\times10^{4}}
\@namedef{num@full.ho.mse.gainmin.1000}{5.8}
\@namedef{num@full.ho.mse.gainmin.10000}{26}
\@namedef{num@full.ho.mse.gainmin.100000}{1.7}
\@namedef{num@full.ho.mse.units.1000}{6}
\@namedef{num@full.ho.mse.units.10000}{6}
\@namedef{num@full.ho.mse.units.100000}{6}
\@namedef{num@full.ho.mse.wins.1000}{5}
\@namedef{num@full.ho.mse.wins.10000}{6}
\@namedef{num@full.ho.mse.wins.100000}{6}
\@namedef{num@full.ho.unexpl.gainmax.1000}{3.1\times10^{6}}
\@namedef{num@full.ho.unexpl.gainmax.10000}{1.3\times10^{5}}
\@namedef{num@full.ho.unexpl.gainmax.100000}{9.1\times10^{4}}
\@namedef{num@full.ho.unexpl.gainmin.1000}{1.8}
\@namedef{num@full.ho.unexpl.gainmin.10000}{1.4}
\@namedef{num@full.ho.unexpl.gainmin.100000}{1.4}
\@namedef{num@full.ho.unexpl.units.1000}{6}
\@namedef{num@full.ho.unexpl.units.10000}{6}
\@namedef{num@full.ho.unexpl.units.100000}{6}
\@namedef{num@full.ho.unexpl.wins.1000}{6}
\@namedef{num@full.ho.unexpl.wins.10000}{5}
\@namedef{num@full.ho.unexpl.wins.100000}{6}
\@namedef{num@full.hx.bcnf.1000}{85}
\@namedef{num@full.hx.bcnf.10000}{85}
\@namedef{num@full.hx.bcnf.100000}{85}
\@namedef{num@full.hx.bentlogistic.1000}{47}
\@namedef{num@full.hx.bentlogistic.10000}{47}
\@namedef{num@full.hx.bentlogistic.100000}{47}
\@namedef{num@full.hx.curvedtent.1000}{68}
\@namedef{num@full.hx.curvedtent.10000}{68}
\@namedef{num@full.hx.curvedtent.100000}{68}
\@namedef{num@full.hx.henon.10000}{78}
\@namedef{num@full.hx.henon.100000}{78}
\@namedef{num@full.hx.lozi.1000}{74}
\@namedef{num@full.hx.lozi.10000}{74}
\@namedef{num@full.hx.lozi.100000}{74}
\@namedef{num@full.hx.quadtent.1000}{57}
\@namedef{num@full.hx.quadtent.10000}{57}
\@namedef{num@full.hx.quadtent.100000}{57}
\@namedef{num@full.hx.series1.1000}{more than 20{,}000 (1.00)}
\@namedef{num@full.hx.series1.10000}{more than 20{,}000 (1.00)}
\@namedef{num@full.hx.series1.100000}{more than 20{,}000 (1.00)}
\@namedef{num@full.hx.series2.1000}{70}
\@namedef{num@full.hx.series2.10000}{70}
\@namedef{num@full.hx.series2.100000}{70}
\@namedef{num@full.hx.series3.1000}{48}
\@namedef{num@full.hx.series3.10000}{48}
\@namedef{num@full.hx.series3.100000}{48}
\@namedef{num@full.hx.series4.1000}{39}
\@namedef{num@full.hx.series4.10000}{39}
\@namedef{num@full.hx.series4.100000}{39}
\@namedef{num@full.hx.series5.1000}{31}
\@namedef{num@full.hx.series5.10000}{31}
\@namedef{num@full.hx.series5.100000}{31}
\@namedef{num@full.hx.series6.1000}{26}
\@namedef{num@full.hx.series6.10000}{26}
\@namedef{num@full.hx.series6.100000}{26}
\@namedef{num@full.hx.skewtent.1000}{56}
\@namedef{num@full.hx.skewtent.10000}{56}
\@namedef{num@full.hx.skewtent.100000}{56}
\@namedef{num@full.hz.atleast.1000}{11}
\@namedef{num@full.hz.atleast.10000}{11}
\@namedef{num@full.hz.atleast.100000}{12}
\@namedef{num@full.hz.max.1000}{6}
\@namedef{num@full.hz.max.10000}{9}
\@namedef{num@full.hz.max.100000}{11}
\@namedef{num@full.hz.min.1000}{0}
\@namedef{num@full.hz.min.10000}{-1}
\@namedef{num@full.hz.min.100000}{0}
\@namedef{num@full.hz.units.1000}{11}
\@namedef{num@full.hz.units.10000}{12}
\@namedef{num@full.hz.units.100000}{12}
\@namedef{num@full.learn.mse.kgain.max.1000}{6.7\times10^{6}}
\@namedef{num@full.learn.mse.kgain.max.10000}{3.7\times10^{2}}
\@namedef{num@full.learn.mse.kgain.max.100000}{2.2}
\@namedef{num@full.learn.mse.kgain.min.1000}{5.1\times10^{5}}
\@namedef{num@full.learn.mse.kgain.min.10000}{1.1}
\@namedef{num@full.learn.mse.kgain.min.100000}{1.7}
\@namedef{num@full.learn.mse.units.1000}{6}
\@namedef{num@full.learn.mse.units.10000}{6}
\@namedef{num@full.learn.mse.units.100000}{6}
\@namedef{num@full.learn.mse.wins.1000}{5}
\@namedef{num@full.learn.mse.wins.10000}{4}
\@namedef{num@full.learn.mse.wins.100000}{3}
\@namedef{num@full.learn.mse.worst}{1.5}
\@namedef{num@full.learn.mse.worst.1000}{1.4}
\@namedef{num@full.learn.mse.worst.10000}{1.1}
\@namedef{num@full.learn.mse.worst.100000}{1.5}
\@namedef{num@full.learn.unexpl.kgain.max.1000}{1.6}
\@namedef{num@full.learn.unexpl.kgain.max.10000}{2.1}
\@namedef{num@full.learn.unexpl.kgain.max.100000}{1.9}
\@namedef{num@full.learn.unexpl.kgain.min.1000}{1}
\@namedef{num@full.learn.unexpl.kgain.min.10000}{1}
\@namedef{num@full.learn.unexpl.kgain.min.100000}{1.1}
\@namedef{num@full.learn.unexpl.units.1000}{6}
\@namedef{num@full.learn.unexpl.units.10000}{6}
\@namedef{num@full.learn.unexpl.units.100000}{6}
\@namedef{num@full.learn.unexpl.wins.1000}{5}
\@namedef{num@full.learn.unexpl.wins.10000}{5}
\@namedef{num@full.learn.unexpl.wins.100000}{4}
\@namedef{num@full.learn.unexpl.worst}{3.4}
\@namedef{num@full.learn.unexpl.worst.1000}{1.1}
\@namedef{num@full.learn.unexpl.worst.10000}{3.4}
\@namedef{num@full.learn.unexpl.worst.100000}{2.8}
\@namedef{num@full.ratio.argmax.1000}{bentlogistic}
\@namedef{num@full.ratio.argmax.10000}{skewtent}
\@namedef{num@full.ratio.argmax.100000}{curvedtent}
\@namedef{num@full.ratio.bcnf.1000}{1.53}
\@namedef{num@full.ratio.bcnf.10000}{0.90}
\@namedef{num@full.ratio.bcnf.100000}{0.57}
\@namedef{num@full.ratio.below.1000}{4}
\@namedef{num@full.ratio.below.10000}{12}
\@namedef{num@full.ratio.below.100000}{13}
\@namedef{num@full.ratio.bentlogistic.1000}{3.09}
\@namedef{num@full.ratio.bentlogistic.10000}{0.68}
\@namedef{num@full.ratio.bentlogistic.100000}{0.41}
\@namedef{num@full.ratio.curvedtent.1000}{1.15}
\@namedef{num@full.ratio.curvedtent.10000}{1.00}
\@namedef{num@full.ratio.curvedtent.100000}{0.90}
\@namedef{num@full.ratio.henon.10000}{0.20}
\@namedef{num@full.ratio.henon.100000}{0.15}
\@namedef{num@full.ratio.k.max.1000}{1.19}
\@namedef{num@full.ratio.k.max.10000}{0.94}
\@namedef{num@full.ratio.k.max.100000}{0.58}
\@namedef{num@full.ratio.lozi.1000}{1.05}
\@namedef{num@full.ratio.lozi.10000}{0.85}
\@namedef{num@full.ratio.lozi.100000}{0.72}
\@namedef{num@full.ratio.max.1000}{3.09}
\@namedef{num@full.ratio.max.10000}{1.01}
\@namedef{num@full.ratio.max.100000}{0.90}
\@namedef{num@full.ratio.median.1000}{1.11}
\@namedef{num@full.ratio.median.10000}{0.85}
\@namedef{num@full.ratio.median.100000}{0.51}
\@namedef{num@full.ratio.quadtent.1000}{1.23}
\@namedef{num@full.ratio.quadtent.10000}{1.00}
\@namedef{num@full.ratio.quadtent.100000}{0.41}
\@namedef{num@full.ratio.second.1000}{1.53}
\@namedef{num@full.ratio.second.10000}{1.00}
\@namedef{num@full.ratio.second.100000}{0.72}
\@namedef{num@full.ratio.series1.1000}{0.17}
\@namedef{num@full.ratio.series1.10000}{0.07}
\@namedef{num@full.ratio.series1.100000}{0.04}
\@namedef{num@full.ratio.series2.1000}{0.37}
\@namedef{num@full.ratio.series2.10000}{0.33}
\@namedef{num@full.ratio.series2.100000}{0.32}
\@namedef{num@full.ratio.series3.1000}{0.35}
\@namedef{num@full.ratio.series3.10000}{0.32}
\@namedef{num@full.ratio.series3.100000}{0.30}
\@namedef{num@full.ratio.series4.1000}{1.07}
\@namedef{num@full.ratio.series4.10000}{0.83}
\@namedef{num@full.ratio.series4.100000}{0.54}
\@namedef{num@full.ratio.series5.1000}{0.76}
\@namedef{num@full.ratio.series5.10000}{0.94}
\@namedef{num@full.ratio.series5.100000}{0.51}
\@namedef{num@full.ratio.series6.1000}{1.19}
\@namedef{num@full.ratio.series6.10000}{0.85}
\@namedef{num@full.ratio.series6.100000}{0.58}
\@namedef{num@full.ratio.skewtent.1000}{1.18}
\@namedef{num@full.ratio.skewtent.10000}{1.01}
\@namedef{num@full.ratio.skewtent.100000}{0.72}
\@namedef{num@full.ratio.units.1000}{12}
\@namedef{num@full.ratio.units.10000}{13}
\@namedef{num@full.ratio.units.100000}{13}
\@namedef{num@full.sf.100}{1.00}
\@namedef{num@full.sf.25}{0.0018}
\@namedef{num@full.sf.50}{0.111}
\@namedef{num@full.sf.m}{8}
\@namedef{num@noise.full.cells}{18}
\@namedef{num@noise.full.gain0.max}{2.4}
\@namedef{num@noise.full.gain0.min}{1.7}
\@namedef{num@noise.full.gainhi.max}{10}
\@namedef{num@noise.full.s2.max}{1.03}
\@namedef{num@noise.full.s2.min}{0.99}
\@namedef{num@noise.full.wins}{18}
\makeatother


==> tables/kink_numbers.tex <==
% written by experiments/paper_figures/kink_band.py from the confirmation's stored per-point errors
\makeatletter\@namedef{num@kb.units}{32}\makeatother
\makeatletter\@namedef{num@kb.cs.median}{1}\makeatother
\makeatletter\@namedef{num@kb.base.median}{93}\makeatother
\makeatletter\@namedef{num@kb.base.min}{0}\makeatother
\makeatletter\@namedef{num@kb.base.max}{100}\makeatother
\makeatletter\@namedef{num@kb.cs.min}{0}\makeatother
\makeatletter\@namedef{num@kb.cs.max}{4}\makeatother
\makeatletter\@namedef{num@kb.base.majority}{25}\makeatother
\makeatletter\@namedef{num@kb.cs.majority}{0}\makeatother


==> tables/noise_transition_numbers.tex <==
% written by experiments/csf_noise/analyse_noise.py from the noise-transition results
\makeatletter\@namedef{num@nt.h1.cells}{36}\makeatother
\makeatletter\@namedef{num@nt.h1.within}{35}\makeatother
\makeatletter\@namedef{num@nt.h1.min}{0.67}\makeatother
\makeatletter\@namedef{num@nt.h1.max}{1.73}\makeatother
\makeatletter\@namedef{num@nt.h1.verdict}{failed}\makeatother
\makeatletter\@namedef{num@nt.h1.fail.system}{Lozi}\makeatother
\makeatletter\@namedef{num@nt.h1.fail.n}{10^{3}}\makeatother
\makeatletter\@namedef{num@nt.h1.fail.eps}{10^{-3}}\makeatother
\makeatletter\@namedef{num@nt.h1.fail.ratio}{1.73}\makeatother
\makeatletter\@namedef{num@nt.h1.fail.count}{1}\makeatother
\makeatletter\@namedef{num@nt.h2.ok}{5}\makeatother
\makeatletter\@namedef{num@nt.h2.verdict}{held}\makeatother
\makeatletter\@namedef{num@nt.h2.big}{10^{-7}}\makeatother
\makeatletter\@namedef{num@nt.h2.small.min}{10^{-7}}\makeatother
\makeatletter\@namedef{num@nt.h2.small.max}{10^{-2}}\makeatother
\makeatletter\@namedef{num@nt.h3.part1}{3}\makeatother
\makeatletter\@namedef{num@nt.h3.verdict}{failed}\makeatother
\makeatletter\@namedef{num@nt.h3.cs.max.system}{Border collision}\makeatother
\makeatletter\@namedef{num@nt.h3.cs.series4}{99}\makeatother
\makeatletter\@namedef{num@nt.h3.cs.bcnf}{100}\makeatother
\makeatletter\@namedef{num@nt.h3.base.bcnf}{98}\makeatother
\makeatletter\@namedef{num@nt.h3.over.n}{1}\makeatother
\makeatletter\@namedef{num@nt.h3.over.system}{Border collision}\makeatother
\makeatletter\@namedef{num@nt.h3.over.method}{S-map}\makeatother
\makeatletter\@namedef{num@nt.h3.over.share}{22}\makeatother
\makeatletter\@namedef{num@nt.h3.others.max}{9.1}\makeatother
\makeatletter\@namedef{num@nt.below.exact}{23}\makeatother
\makeatletter\@namedef{num@nt.below.cells}{24}\makeatother
\makeatletter\@namedef{num@nt.jobs}{126}\makeatother


==> tables/numbers.tex <==
% generated by paper/tables_v3.py from the v3 results -- do not edit
\makeatletter
\@namedef{num@abl.2.full}{4.4\times10^{-16}}
\@namedef{num@abl.2.kmeansinit}{4.4\times10^{-16}}
\@namedef{num@abl.2.m1}{1.5\times10^{-15}}
\@namedef{num@abl.2.nodensify}{4.4\times10^{-16}}
\@namedef{num@abl.2.notrend}{4.5\times10^{-16}}
\@namedef{num@abl.2.trendonly}{4.4\times10^{-16}}
\@namedef{num@abl.2.uniforminit}{4.4\times10^{-16}}
\@namedef{num@abl.3.full}{4.1\times10^{-16}}
\@namedef{num@abl.3.kmeansinit}{4.1\times10^{-16}}
\@namedef{num@abl.3.m1}{1.4\times10^{-15}}
\@namedef{num@abl.3.nodensify}{4.1\times10^{-16}}
\@namedef{num@abl.3.notrend}{4.2\times10^{-16}}
\@namedef{num@abl.3.trendonly}{4.1\times10^{-16}}
\@namedef{num@abl.3.uniforminit}{4.1\times10^{-16}}
\@namedef{num@abl.4.full}{2.3\times10^{-13}}
\@namedef{num@abl.4.kmeansinit}{2.5\times10^{-12}}
\@namedef{num@abl.4.m1}{4.1\times10^{-15}}
\@namedef{num@abl.4.nodensify}{3.1\times10^{-7}}
\@namedef{num@abl.4.notrend}{2.3\times10^{-13}}
\@namedef{num@abl.4.trendonly}{8.2\times10^{-5}}
\@namedef{num@abl.4.uniforminit}{7.5\times10^{-13}}
\@namedef{num@abl.5.full}{5.9\times10^{-10}}
\@namedef{num@abl.5.kmeansinit}{1.7\times10^{-11}}
\@namedef{num@abl.5.m1}{1.5\times10^{-14}}
\@namedef{num@abl.5.nodensify}{8.0\times10^{-7}}
\@namedef{num@abl.5.notrend}{5.9\times10^{-10}}
\@namedef{num@abl.5.trendonly}{7.3\times10^{-4}}
\@namedef{num@abl.5.uniforminit}{5.5\times10^{-12}}
\@namedef{num@abl.6.full}{2.1\times10^{-13}}
\@namedef{num@abl.6.kmeansinit}{1.4\times10^{-14}}
\@namedef{num@abl.6.m1}{2.1\times10^{-13}}
\@namedef{num@abl.6.nodensify}{8.9\times10^{-9}}
\@namedef{num@abl.6.notrend}{7.3\times10^{-12}}
\@namedef{num@abl.6.trendonly}{3.0\times10^{-3}}
\@namedef{num@abl.6.uniforminit}{6.6\times10^{-15}}
\@namedef{num@abl.henon.full}{7.2\times10^{-16}}
\@namedef{num@abl.henon.kmeansinit}{7.3\times10^{-16}}
\@namedef{num@abl.henon.m1}{3.7\times10^{-2}}
\@namedef{num@abl.henon.nodensify}{7.2\times10^{-16}}
\@namedef{num@abl.henon.notrend}{8.0\times10^{-16}}
\@namedef{num@abl.henon.trendonly}{7.3\times10^{-16}}
\@namedef{num@abl.henon.uniforminit}{7.2\times10^{-16}}
\@namedef{num@abl.kinked.nodensify.max}{8.0\times10^{-7}}
\@namedef{num@abl.kinked.nodensify.min}{8.9\times10^{-9}}
\@namedef{num@abl.smooth.series}{2, 3}
\@namedef{num@abl.smooth.spread}{11}
\@namedef{num@ci.2.best}{Local polynomial, own window}
\@namedef{num@ci.2.best20}{Local polynomial, own window}
\@namedef{num@ci.2.csclosershare}{49}
\@namedef{num@ci.2.cstop1pctshareofsse}{11}
\@namedef{num@ci.2.hi}{0.99}
\@namedef{num@ci.2.hi20}{0.92}
\@namedef{num@ci.2.lo}{0.98}
\@namedef{num@ci.2.lo20}{0.76}
\@namedef{num@ci.2.ratio}{0.98}
\@namedef{num@ci.2.ratio20}{0.84}
\@namedef{num@ci.3.best}{Local polynomial}
\@namedef{num@ci.3.best20}{Local polynomial}
\@namedef{num@ci.3.csclosershare}{49}
\@namedef{num@ci.3.cstop1pctshareofsse}{14}
\@namedef{num@ci.3.hi}{0.99}
\@namedef{num@ci.3.hi20}{1.10}
\@namedef{num@ci.3.lo}{0.99}
\@namedef{num@ci.3.lo20}{0.86}
\@namedef{num@ci.3.ratio}{0.99}
\@namedef{num@ci.3.ratio20}{0.97}
\@namedef{num@ci.4.best}{S-map}
\@namedef{num@ci.4.best20}{Local polynomial}
\@namedef{num@ci.4.csclosershare}{59}
\@namedef{num@ci.4.csssesharekinkband}{48}
\@namedef{num@ci.4.cstop1pctshareofsse}{55}
\@namedef{num@ci.4.hi}{1.91}
\@namedef{num@ci.4.hi20}{1.32}
\@namedef{num@ci.4.kinkbandsharepoints}{1}
\@namedef{num@ci.4.lo}{0.50}
\@namedef{num@ci.4.lo20}{1.17}
\@namedef{num@ci.4.localssesharekinkband}{8}
\@namedef{num@ci.4.ratio}{0.96}
\@namedef{num@ci.4.ratio20}{1.24}
\@namedef{num@ci.5.best}{S-map}
\@namedef{num@ci.5.best20}{Local polynomial}
\@namedef{num@ci.5.csclosershare}{56}
\@namedef{num@ci.5.csssesharekinkband}{91}
\@namedef{num@ci.5.cstop1pctshareofsse}{92}
\@namedef{num@ci.5.hi}{3.13}
\@namedef{num@ci.5.hi20}{1.02}
\@namedef{num@ci.5.kinkbandsharepoints}{1}
\@namedef{num@ci.5.lo}{0.05}
\@namedef{num@ci.5.lo20}{0.98}
\@namedef{num@ci.5.localssesharekinkband}{44}
\@namedef{num@ci.5.ratio}{0.22}
\@namedef{num@ci.5.ratio20}{1.00}
\@namedef{num@ci.6.best}{S-map}
\@namedef{num@ci.6.best20}{S-map}
\@namedef{num@ci.6.csclosershare}{56}
\@namedef{num@ci.6.csssesharekinkband}{13}
\@namedef{num@ci.6.cstop1pctshareofsse}{19}
\@namedef{num@ci.6.hi}{1.26}
\@namedef{num@ci.6.hi20}{1.03}
\@namedef{num@ci.6.kinkbandsharepoints}{1}
\@namedef{num@ci.6.lo}{1.10}
\@namedef{num@ci.6.lo20}{0.99}
\@namedef{num@ci.6.localssesharekinkband}{8}
\@namedef{num@ci.6.ratio}{1.19}
\@namedef{num@ci.6.ratio20}{1.01}
\@namedef{num@cost.bcnf.1000.cs.us}{1.1}
\@namedef{num@cost.bcnf.1000.esn.us}{1.6e+03}
\@namedef{num@cost.bcnf.1000.exact.us}{0.0089}
\@namedef{num@cost.bcnf.1000.lp.us}{12}
\@namedef{num@cost.bcnf.1000.ngrc.us}{0.4}
\@namedef{num@cost.bcnf.1000.poly.us}{0.65}
\@namedef{num@cost.bcnf.1000.smap.us}{9.2}
\@namedef{num@cost.bcnf.10000.cs.us}{1.1}
\@namedef{num@cost.bcnf.10000.esn.us}{1.7e+03}
\@namedef{num@cost.bcnf.10000.exact.us}{0.0097}
\@namedef{num@cost.bcnf.10000.lp.us}{3.7}
\@namedef{num@cost.bcnf.10000.ngrc.us}{0.39}
\@namedef{num@cost.bcnf.10000.poly.us}{0.25}
\@namedef{num@cost.bcnf.10000.rbf.us}{1.1e+02}
\@namedef{num@cost.bcnf.10000.smap.us}{6.9}
\@namedef{num@cost.bcnf.100000.cs.us}{0.95}
\@namedef{num@cost.bcnf.100000.esn.us}{1.8e+03}
\@namedef{num@cost.bcnf.100000.exact.us}{0.0085}
\@namedef{num@cost.bcnf.100000.lp.us}{12}
\@namedef{num@cost.bcnf.100000.ngrc.us}{1.6}
\@namedef{num@cost.bcnf.100000.poly.us}{0.25}
\@namedef{num@cost.bcnf.100000.rbf.us}{94}
\@namedef{num@cost.bcnf.100000.smap.us}{6.8}
\@namedef{num@cost.bcnf.900000.cs.us}{1}
\@namedef{num@cost.bcnf.900000.exact.us}{0.0088}
\@namedef{num@cost.bcnf.900000.lp.us}{5.4}
\@namedef{num@cost.bcnf.900000.ngrc.us}{2.6}
\@namedef{num@cost.bcnf.900000.poly.us}{0.68}
\@namedef{num@cost.bcnf.900000.rbf.us}{1.2e+02}
\@namedef{num@cost.bcnf.900000.smap.us}{13}
\@namedef{num@cost.lozi.1000.cs.us}{0.81}
\@namedef{num@cost.lozi.1000.esn.us}{1.8e+03}
\@namedef{num@cost.lozi.1000.exact.us}{0.0035}
\@namedef{num@cost.lozi.1000.lp.us}{6.8}
\@namedef{num@cost.lozi.1000.ngrc.us}{0.38}
\@namedef{num@cost.lozi.1000.poly.us}{0.25}
\@namedef{num@cost.lozi.1000.smap.us}{9.3}
\@namedef{num@cost.lozi.10000.cs.us}{1.1}
\@namedef{num@cost.lozi.10000.esn.us}{1.7e+03}
\@namedef{num@cost.lozi.10000.exact.us}{0.0038}
\@namedef{num@cost.lozi.10000.lp.us}{3.1}
\@namedef{num@cost.lozi.10000.ngrc.us}{0.67}
\@namedef{num@cost.lozi.10000.poly.us}{0.26}
\@namedef{num@cost.lozi.10000.rbf.us}{97}
\@namedef{num@cost.lozi.10000.smap.us}{4.5}
\@namedef{num@cost.lozi.100000.cs.us}{1}
\@namedef{num@cost.lozi.100000.esn.us}{1.6e+03}
\@namedef{num@cost.lozi.100000.exact.us}{0.0037}
\@namedef{num@cost.lozi.100000.lp.us}{10}
\@namedef{num@cost.lozi.100000.ngrc.us}{0.65}
\@namedef{num@cost.lozi.100000.poly.us}{0.26}
\@namedef{num@cost.lozi.100000.rbf.us}{97}
\@namedef{num@cost.lozi.100000.smap.us}{11}
\@namedef{num@cost.lozi.900000.cs.us}{0.92}
\@namedef{num@cost.lozi.900000.exact.us}{0.0037}
\@namedef{num@cost.lozi.900000.lp.us}{4.2}
\@namedef{num@cost.lozi.900000.ngrc.us}{1.6}
\@namedef{num@cost.lozi.900000.poly.us}{0.27}
\@namedef{num@cost.lozi.900000.rbf.us}{97}
\@namedef{num@cost.lozi.900000.smap.us}{7}
\@namedef{num@cost.skewtent.1000.cs.us}{0.76}
\@namedef{num@cost.skewtent.1000.esn.us}{1.7e+03}
\@namedef{num@cost.skewtent.1000.exact.us}{0.0057}
\@namedef{num@cost.skewtent.1000.lp.us}{3.1}
\@namedef{num@cost.skewtent.1000.ngrc.us}{0.22}
\@namedef{num@cost.skewtent.1000.poly.us}{0.069}
\@namedef{num@cost.skewtent.1000.smap.us}{4.7}
\@namedef{num@cost.skewtent.10000.cs.us}{0.58}
\@namedef{num@cost.skewtent.10000.esn.us}{1.7e+03}
\@namedef{num@cost.skewtent.10000.exact.us}{0.0066}
\@namedef{num@cost.skewtent.10000.lp.us}{2.4}
\@namedef{num@cost.skewtent.10000.ngrc.us}{0.095}
\@namedef{num@cost.skewtent.10000.poly.us}{0.063}
\@namedef{num@cost.skewtent.10000.rbf.us}{42}
\@namedef{num@cost.skewtent.10000.smap.us}{2.6}
\@namedef{num@cost.skewtent.100000.cs.us}{0.66}
\@namedef{num@cost.skewtent.100000.esn.us}{1.7e+03}
\@namedef{num@cost.skewtent.100000.exact.us}{0.0062}
\@namedef{num@cost.skewtent.100000.lp.us}{2.6}
\@namedef{num@cost.skewtent.100000.ngrc.us}{0.056}
\@namedef{num@cost.skewtent.100000.poly.us}{0.068}
\@namedef{num@cost.skewtent.100000.rbf.us}{37}
\@namedef{num@cost.skewtent.100000.smap.us}{5.9}
\@namedef{num@cost.skewtent.900000.cs.us}{1.3}
\@namedef{num@cost.skewtent.900000.exact.us}{0.0067}
\@namedef{num@cost.skewtent.900000.lp.us}{10}
\@namedef{num@cost.skewtent.900000.ngrc.us}{0.42}
\@namedef{num@cost.skewtent.900000.poly.us}{0.3}
\@namedef{num@cost.skewtent.900000.rbf.us}{94}
\@namedef{num@cost.skewtent.900000.smap.us}{27}
\@namedef{num@dy.Lorenz.cs}{0.729}
\@namedef{num@dy.Lorenz.n}{16}
\@namedef{num@dy.Lorenz.poly}{0.729}
\@namedef{num@dy.Lorenz.rank}{1}
\@namedef{num@dy.Lorenz96.cs}{11.2}
\@namedef{num@dy.Lorenz96.n}{16}
\@namedef{num@dy.Lorenz96.poly}{13.0}
\@namedef{num@dy.Lorenz96.rank}{1}
\@namedef{num@dy.MackeyGlass.cs}{6.31}
\@namedef{num@dy.MackeyGlass.n}{16}
\@namedef{num@dy.MackeyGlass.rank}{10}
\@namedef{num@dy.Rossler.cs}{0.112}
\@namedef{num@dy.Rossler.n}{16}
\@namedef{num@dy.Rossler.poly}{0.0573}
\@namedef{num@dy.Rossler.rank}{1}
\@namedef{num@f32.max}{114}
\@namedef{num@f32.min}{1.3}
\@namedef{num@henon.best.mse}{6.8\times10^{-16}}
\@namedef{num@henon.best.name}{Local polynomial, own window}
\@namedef{num@henon.best.ratiofloor}{1.6}
\@namedef{num@henon.best20.name}{Local polynomial, own window}
\@namedef{num@henon.best20.un}{6.0\times10^{-9}}
\@namedef{num@henon.cs.m}{6}
\@namedef{num@henon.cs.mse}{7.2\times10^{-16}}
\@namedef{num@henon.cs.size}{7.4\times10^{3}}
\@namedef{num@henon.cs.splats}{184}
\@namedef{num@henon.cs.un}{7.6\times10^{-9}}
\@namedef{num@henon.esn.m}{6}
\@namedef{num@henon.esn.mse}{4.0\times10^{-15}}
\@namedef{num@henon.esn.un}{1.4\times10^{-7}}
\@namedef{num@henon.exact.mse}{4.1\times10^{-15}}
\@namedef{num@henon.exact.un}{1.6\times10^{-7}}
\@namedef{num@henon.floor.mse}{4.3\times10^{-16}}
\@namedef{num@henon.lpo.m}{9}
\@namedef{num@henon.lpo.mse}{6.8\times10^{-16}}
\@namedef{num@henon.lpo.un}{6.0\times10^{-9}}
\@namedef{num@henon.ngrc.m}{6}
\@namedef{num@henon.ngrc.mse}{2.4\times10^{-15}}
\@namedef{num@henon.ngrc.un}{7.4\times10^{-8}}
\@namedef{num@henon.poly.m}{6}
\@namedef{num@henon.poly.mse}{7.8\times10^{-16}}
\@namedef{num@henon.poly.un}{8.0\times10^{-9}}
\@namedef{num@henon.ratio}{0.94}
\@namedef{num@henon.ratio20}{0.79}
\@namedef{num@henon.ratioexact}{0.18}
\@namedef{num@henon.ratiofloor}{1.7}
\@namedef{num@henon.ratioglobal}{1}
\@namedef{num@henon.smapo.m}{2}
\@namedef{num@henon.smapo.mse}{6.0\times10^{-15}}
\@namedef{num@henon.smapo.un}{2.4\times10^{-7}}
\@namedef{num@ho.H1.cells}{6}
\@namedef{num@ho.H1.lossmax}{115}
\@namedef{num@ho.H1.lossmin}{3.7}
\@namedef{num@ho.H1.verdict}{fails}
\@namedef{num@ho.H1.wins}{2}
\@namedef{num@ho.H2.verdict}{fails}
\@namedef{num@ho.H3.max}{3\times10^{11}}
\@namedef{num@ho.H3.min}{2\times10^{9}}
\@namedef{num@ho.H3.verdict}{holds}
\@namedef{num@ho.bcnf.1000.best.mse}{8.3\times10^{-8}}
\@namedef{num@ho.bcnf.1000.best.msename}{S-map, own window}
\@namedef{num@ho.bcnf.1000.best.un}{2.8\times10^{-2}}
\@namedef{num@ho.bcnf.1000.best.unname}{S-map, own window}
\@namedef{num@ho.bcnf.1000.cs.mse}{6.2\times10^{-7}}
\@namedef{num@ho.bcnf.1000.cs.splats}{209}
\@namedef{num@ho.bcnf.1000.cs.un}{1.4\times10^{-1}}
\@namedef{num@ho.bcnf.1000.exact.mse}{5.0\times10^{-16}}
\@namedef{num@ho.bcnf.1000.exact.un}{4.1\times10^{-9}}
\@namedef{num@ho.bcnf.1000.mse.ratio}{7.4}
\@namedef{num@ho.bcnf.1000.un.ratio}{5}
\@namedef{num@ho.bcnf.10000.best.mse}{5.4\times10^{-11}}
\@namedef{num@ho.bcnf.10000.best.msename}{S-map}
\@namedef{num@ho.bcnf.10000.best.un}{7.7\times10^{-4}}
\@namedef{num@ho.bcnf.10000.best.unname}{S-map}
\@namedef{num@ho.bcnf.10000.cs.mse}{1.9\times10^{-8}}
\@namedef{num@ho.bcnf.10000.cs.splats}{202}
\@namedef{num@ho.bcnf.10000.cs.un}{8.9\times10^{-2}}
\@namedef{num@ho.bcnf.10000.exact.mse}{5.0\times10^{-16}}
\@namedef{num@ho.bcnf.10000.exact.un}{4.1\times10^{-9}}
\@namedef{num@ho.bcnf.10000.mse.ratio}{356}
\@namedef{num@ho.bcnf.10000.un.ratio}{115}
\@namedef{num@ho.bcnf.100000.best.mse}{3.5\times10^{-14}}
\@namedef{num@ho.bcnf.100000.best.msename}{S-map}
\@namedef{num@ho.bcnf.100000.best.un}{1.2\times10^{-4}}
\@namedef{num@ho.bcnf.100000.best.unname}{Local polynomial}
\@namedef{num@ho.bcnf.100000.cs.mse}{1.3\times10^{-11}}
\@namedef{num@ho.bcnf.100000.cs.splats}{627}
\@namedef{num@ho.bcnf.100000.cs.un}{1.2\times10^{-4}}
\@namedef{num@ho.bcnf.100000.exact.mse}{5.0\times10^{-16}}
\@namedef{num@ho.bcnf.100000.exact.un}{4.1\times10^{-9}}
\@namedef{num@ho.bcnf.100000.mse.ratio}{385}
\@namedef{num@ho.bcnf.100000.un.ratio}{0.97}
\@namedef{num@ho.bcnf.900000.best.mse}{6.2\times10^{-16}}
\@namedef{num@ho.bcnf.900000.best.msename}{Local polynomial, own window}
\@namedef{num@ho.bcnf.900000.best.un}{1.1\times10^{-7}}
\@namedef{num@ho.bcnf.900000.best.unname}{S-map, own window}
\@namedef{num@ho.bcnf.900000.cs.mse}{6.8\times10^{-14}}
\@namedef{num@ho.bcnf.900000.cs.splats}{899}
\@namedef{num@ho.bcnf.900000.cs.un}{4.0\times10^{-6}}
\@namedef{num@ho.bcnf.900000.exact.mse}{5.0\times10^{-16}}
\@namedef{num@ho.bcnf.900000.exact.un}{4.1\times10^{-9}}
\@namedef{num@ho.bcnf.900000.mse.ratio}{111}
\@namedef{num@ho.bcnf.900000.un.ratio}{36}
\@namedef{num@ho.bcnf.H2.bestname}{Local polynomial, own window}
\@namedef{num@ho.bcnf.H2.vsbest}{111}
\@namedef{num@ho.bcnf.H2.vsexact}{135}
\@namedef{num@ho.bcnf.Kexp}{0.21}
\@namedef{num@ho.bentlogistic.1000.best.mse}{8.3\times10^{-13}}
\@namedef{num@ho.bentlogistic.1000.best.msename}{Local polynomial}
\@namedef{num@ho.bentlogistic.1000.best.un}{1.9\times10^{-2}}
\@namedef{num@ho.bentlogistic.1000.best.unname}{Local polynomial}
\@namedef{num@ho.bentlogistic.1000.cs.mse}{8.8\times10^{-14}}
\@namedef{num@ho.bentlogistic.1000.cs.splats}{208}
\@namedef{num@ho.bentlogistic.1000.cs.un}{1.2\times10^{-2}}
\@namedef{num@ho.bentlogistic.1000.exact.mse}{1.2\times10^{-15}}
\@namedef{num@ho.bentlogistic.1000.exact.un}{9.0\times10^{-3}}
\@namedef{num@ho.bentlogistic.1000.mse.ratio}{0.11}
\@namedef{num@ho.bentlogistic.1000.un.ratio}{0.63}
\@namedef{num@ho.bentlogistic.10000.best.mse}{2.2\times10^{-14}}
\@namedef{num@ho.bentlogistic.10000.best.msename}{S-map}
\@namedef{num@ho.bentlogistic.10000.best.un}{2.8\times10^{-2}}
\@namedef{num@ho.bentlogistic.10000.best.unname}{S-map}
\@namedef{num@ho.bentlogistic.10000.cs.mse}{3.7\times10^{-15}}
\@namedef{num@ho.bentlogistic.10000.cs.splats}{201}
\@namedef{num@ho.bentlogistic.10000.cs.un}{9.3\times10^{-3}}
\@namedef{num@ho.bentlogistic.10000.exact.mse}{1.2\times10^{-15}}
\@namedef{num@ho.bentlogistic.10000.exact.un}{9.0\times10^{-3}}
\@namedef{num@ho.bentlogistic.10000.mse.ratio}{0.17}
\@namedef{num@ho.bentlogistic.10000.un.ratio}{0.33}
\@namedef{num@ho.bentlogistic.100000.best.mse}{8.8\times10^{-16}}
\@namedef{num@ho.bentlogistic.100000.best.msename}{S-map, own window}
\@namedef{num@ho.bentlogistic.100000.best.un}{1.4\times10^{-3}}
\@namedef{num@ho.bentlogistic.100000.best.unname}{S-map, own window}
\@namedef{num@ho.bentlogistic.100000.cs.mse}{1.2\times10^{-15}}
\@namedef{num@ho.bentlogistic.100000.cs.splats}{320}
\@namedef{num@ho.bentlogistic.100000.cs.un}{9.4\times10^{-3}}
\@namedef{num@ho.bentlogistic.100000.exact.mse}{1.2\times10^{-15}}
\@namedef{num@ho.bentlogistic.100000.exact.un}{9.0\times10^{-3}}
\@namedef{num@ho.bentlogistic.100000.mse.ratio}{1.3}
\@namedef{num@ho.bentlogistic.100000.un.ratio}{6.9}
\@namedef{num@ho.bentlogistic.900000.best.mse}{5.5\times10^{-16}}
\@namedef{num@ho.bentlogistic.900000.best.msename}{Local polynomial}
\@namedef{num@ho.bentlogistic.900000.best.un}{6.0\times10^{-4}}
\@namedef{num@ho.bentlogistic.900000.best.unname}{Local polynomial}
\@namedef{num@ho.bentlogistic.900000.cs.mse}{6.0\times10^{-16}}
\@namedef{num@ho.bentlogistic.900000.cs.splats}{506}
\@namedef{num@ho.bentlogistic.900000.cs.un}{6.8\times10^{-5}}
\@namedef{num@ho.bentlogistic.900000.exact.mse}{1.2\times10^{-15}}
\@namedef{num@ho.bentlogistic.900000.exact.un}{9.0\times10^{-3}}
\@namedef{num@ho.bentlogistic.900000.mse.ratio}{1.1}
\@namedef{num@ho.bentlogistic.900000.un.ratio}{0.11}
\@namedef{num@ho.bentlogistic.H2.bestname}{Local polynomial}
\@namedef{num@ho.bentlogistic.H2.vsbest}{1.1}
\@namedef{num@ho.bentlogistic.H2.vsexact}{0.52}
\@namedef{num@ho.curvedtent.1000.best.mse}{9.8\times10^{-10}}
\@namedef{num@ho.curvedtent.1000.best.msename}{S-map}
\@namedef{num@ho.curvedtent.1000.best.un}{9.0\times10^{-2}}
\@namedef{num@ho.curvedtent.1000.best.unname}{Local polynomial}
\@namedef{num@ho.curvedtent.1000.cs.mse}{4.5\times10^{-3}}
\@namedef{num@ho.curvedtent.1000.cs.splats}{201}
\@namedef{num@ho.curvedtent.1000.cs.un}{1.2\times10^{-1}}
\@namedef{num@ho.curvedtent.1000.exact.mse}{8.9\times10^{-16}}
\@namedef{num@ho.curvedtent.1000.exact.un}{1.3\times10^{-3}}
\@namedef{num@ho.curvedtent.1000.mse.ratio}{4616558}
\@namedef{num@ho.curvedtent.1000.un.ratio}{1.4}
\@namedef{num@ho.curvedtent.10000.best.mse}{4.3\times10^{-14}}
\@namedef{num@ho.curvedtent.10000.best.msename}{Local polynomial}
\@namedef{num@ho.curvedtent.10000.best.un}{2.7\times10^{-3}}
\@namedef{num@ho.curvedtent.10000.best.unname}{Local polynomial}
\@namedef{num@ho.curvedtent.10000.cs.mse}{1.9\times10^{-11}}
\@namedef{num@ho.curvedtent.10000.cs.splats}{249}
\@namedef{num@ho.curvedtent.10000.cs.un}{1.3\times10^{-3}}
\@namedef{num@ho.curvedtent.10000.exact.mse}{8.9\times10^{-16}}
\@namedef{num@ho.curvedtent.10000.exact.un}{1.3\times10^{-3}}
\@namedef{num@ho.curvedtent.10000.mse.ratio}{456}
\@namedef{num@ho.curvedtent.10000.un.ratio}{0.5}
\@namedef{num@ho.curvedtent.100000.best.mse}{1.4\times10^{-15}}
\@namedef{num@ho.curvedtent.100000.best.msename}{Local polynomial}
\@namedef{num@ho.curvedtent.100000.best.un}{1.5\times10^{-3}}
\@namedef{num@ho.curvedtent.100000.best.unname}{Local polynomial}
\@namedef{num@ho.curvedtent.100000.cs.mse}{9.2\times10^{-16}}
\@namedef{num@ho.curvedtent.100000.cs.splats}{379}
\@namedef{num@ho.curvedtent.100000.cs.un}{1.3\times10^{-3}}
\@namedef{num@ho.curvedtent.100000.exact.mse}{8.9\times10^{-16}}
\@namedef{num@ho.curvedtent.100000.exact.un}{1.3\times10^{-3}}
\@namedef{num@ho.curvedtent.100000.mse.ratio}{0.67}
\@namedef{num@ho.curvedtent.100000.un.ratio}{0.85}
\@namedef{num@ho.curvedtent.900000.best.mse}{1.0\times10^{-15}}
\@namedef{num@ho.curvedtent.900000.best.msename}{Local polynomial}
\@namedef{num@ho.curvedtent.900000.best.un}{1.5\times10^{-3}}
\@namedef{num@ho.curvedtent.900000.best.unname}{Local polynomial}
\@namedef{num@ho.curvedtent.900000.cs.mse}{8.9\times10^{-16}}
\@namedef{num@ho.curvedtent.900000.cs.splats}{368}
\@namedef{num@ho.curvedtent.900000.cs.un}{1.3\times10^{-3}}
\@namedef{num@ho.curvedtent.900000.exact.mse}{8.9\times10^{-16}}
\@namedef{num@ho.curvedtent.900000.exact.un}{1.3\times10^{-3}}
\@namedef{num@ho.curvedtent.900000.mse.ratio}{0.86}
\@namedef{num@ho.curvedtent.900000.un.ratio}{0.87}
\@namedef{num@ho.curvedtent.H2.bestname}{Local polynomial}
\@namedef{num@ho.curvedtent.H2.vsbest}{0.86}
\@namedef{num@ho.curvedtent.H2.vsexact}{1.0}
\@namedef{num@ho.lozi.1000.best.mse}{3.2\times10^{-6}}
\@namedef{num@ho.lozi.1000.best.msename}{ESN}
\@namedef{num@ho.lozi.1000.best.un}{8.8\times10^{-2}}
\@namedef{num@ho.lozi.1000.best.unname}{S-map}
\@namedef{num@ho.lozi.1000.cs.mse}{1.3\times10^{-5}}
\@namedef{num@ho.lozi.1000.cs.splats}{285}
\@namedef{num@ho.lozi.1000.cs.un}{3.3\times10^{-1}}
\@namedef{num@ho.lozi.1000.exact.mse}{1.3\times10^{-15}}
\@namedef{num@ho.lozi.1000.exact.un}{1.3\times10^{-7}}
\@namedef{num@ho.lozi.1000.mse.ratio}{4}
\@namedef{num@ho.lozi.1000.un.ratio}{3.7}
\@namedef{num@ho.lozi.10000.best.mse}{2.1\times10^{-8}}
\@namedef{num@ho.lozi.10000.best.msename}{Local polynomial}
\@namedef{num@ho.lozi.10000.best.un}{1.1\times10^{-2}}
\@namedef{num@ho.lozi.10000.best.unname}{S-map}
\@namedef{num@ho.lozi.10000.cs.mse}{1.7\times10^{-7}}
\@namedef{num@ho.lozi.10000.cs.splats}{475}
\@namedef{num@ho.lozi.10000.cs.un}{4.7\times10^{-2}}
\@namedef{num@ho.lozi.10000.exact.mse}{1.3\times10^{-15}}
\@namedef{num@ho.lozi.10000.exact.un}{1.3\times10^{-7}}
\@namedef{num@ho.lozi.10000.mse.ratio}{8}
\@namedef{num@ho.lozi.10000.un.ratio}{4.3}
\@namedef{num@ho.lozi.100000.best.mse}{2.2\times10^{-11}}
\@namedef{num@ho.lozi.100000.best.msename}{S-map}
\@namedef{num@ho.lozi.100000.best.un}{1.9\times10^{-3}}
\@namedef{num@ho.lozi.100000.best.unname}{S-map, own window}
\@namedef{num@ho.lozi.100000.cs.mse}{9.0\times10^{-10}}
\@namedef{num@ho.lozi.100000.cs.splats}{760}
\@namedef{num@ho.lozi.100000.cs.un}{8.7\times10^{-3}}
\@namedef{num@ho.lozi.100000.exact.mse}{1.3\times10^{-15}}
\@namedef{num@ho.lozi.100000.exact.un}{1.3\times10^{-7}}
\@namedef{num@ho.lozi.100000.mse.ratio}{41}
\@namedef{num@ho.lozi.100000.un.ratio}{4.7}
\@namedef{num@ho.lozi.900000.best.mse}{2.8\times10^{-15}}
\@namedef{num@ho.lozi.900000.best.msename}{S-map}
\@namedef{num@ho.lozi.900000.best.un}{3.2\times10^{-4}}
\@namedef{num@ho.lozi.900000.best.unname}{S-map}
\@namedef{num@ho.lozi.900000.cs.mse}{3.6\times10^{-15}}
\@namedef{num@ho.lozi.900000.cs.splats}{1{,}889}
\@namedef{num@ho.lozi.900000.cs.un}{3.0\times10^{-4}}
\@namedef{num@ho.lozi.900000.exact.mse}{1.3\times10^{-15}}
\@namedef{num@ho.lozi.900000.exact.un}{1.3\times10^{-7}}
\@namedef{num@ho.lozi.900000.mse.ratio}{1.3}
\@namedef{num@ho.lozi.900000.un.ratio}{0.95}
\@namedef{num@ho.lozi.H2.bestname}{S-map}
\@namedef{num@ho.lozi.H2.vsbest}{1.3}
\@namedef{num@ho.lozi.H2.vsexact}{2.7}
\@namedef{num@ho.lozi.Kexp}{0.28}
\@namedef{num@ho.quadtent.1000.best.mse}{1.4\times10^{-9}}
\@namedef{num@ho.quadtent.1000.best.msename}{S-map}
\@namedef{num@ho.quadtent.1000.best.un}{2.5\times10^{-2}}
\@namedef{num@ho.quadtent.1000.best.unname}{Local polynomial}
\@namedef{num@ho.quadtent.1000.cs.mse}{2.2\times10^{-10}}
\@namedef{num@ho.quadtent.1000.cs.splats}{194}
\@namedef{num@ho.quadtent.1000.cs.un}{6.6\times10^{-3}}
\@namedef{num@ho.quadtent.1000.exact.mse}{1.1\times10^{-15}}
\@namedef{num@ho.quadtent.1000.exact.un}{3.3\times10^{-6}}
\@namedef{num@ho.quadtent.1000.mse.ratio}{0.16}
\@namedef{num@ho.quadtent.1000.un.ratio}{0.27}
\@namedef{num@ho.quadtent.10000.best.mse}{6.0\times10^{-14}}
\@namedef{num@ho.quadtent.10000.best.msename}{S-map}
\@namedef{num@ho.quadtent.10000.best.un}{3.2\times10^{-4}}
\@namedef{num@ho.quadtent.10000.best.unname}{S-map}
\@namedef{num@ho.quadtent.10000.cs.mse}{8.4\times10^{-13}}
\@namedef{num@ho.quadtent.10000.cs.splats}{202}
\@namedef{num@ho.quadtent.10000.cs.un}{2.1\times10^{-3}}
\@namedef{num@ho.quadtent.10000.exact.mse}{1.1\times10^{-15}}
\@namedef{num@ho.quadtent.10000.exact.un}{3.3\times10^{-6}}
\@namedef{num@ho.quadtent.10000.mse.ratio}{14}
\@namedef{num@ho.quadtent.10000.un.ratio}{6.4}
\@namedef{num@ho.quadtent.100000.best.mse}{9.8\times10^{-16}}
\@namedef{num@ho.quadtent.100000.best.msename}{S-map}
\@namedef{num@ho.quadtent.100000.best.un}{2.8\times10^{-4}}
\@namedef{num@ho.quadtent.100000.best.unname}{S-map}
\@namedef{num@ho.quadtent.100000.cs.mse}{7.8\times10^{-14}}
\@namedef{num@ho.quadtent.100000.cs.splats}{543}
\@namedef{num@ho.quadtent.100000.cs.un}{4.6\times10^{-3}}
\@namedef{num@ho.quadtent.100000.exact.mse}{1.1\times10^{-15}}
\@namedef{num@ho.quadtent.100000.exact.un}{3.3\times10^{-6}}
\@namedef{num@ho.quadtent.100000.mse.ratio}{79}
\@namedef{num@ho.quadtent.100000.un.ratio}{16}
\@namedef{num@ho.quadtent.900000.best.mse}{5.9\times10^{-16}}
\@namedef{num@ho.quadtent.900000.best.msename}{Local polynomial}
\@namedef{num@ho.quadtent.900000.best.un}{6.6\times10^{-7}}
\@namedef{num@ho.quadtent.900000.best.unname}{S-map, own window}
\@namedef{num@ho.quadtent.900000.cs.mse}{6.2\times10^{-16}}
\@namedef{num@ho.quadtent.900000.cs.splats}{883}
\@namedef{num@ho.quadtent.900000.cs.un}{1.5\times10^{-6}}
\@namedef{num@ho.quadtent.900000.exact.mse}{1.1\times10^{-15}}
\@namedef{num@ho.quadtent.900000.exact.un}{3.3\times10^{-6}}
\@namedef{num@ho.quadtent.900000.mse.ratio}{1.1}
\@namedef{num@ho.quadtent.900000.un.ratio}{2.2}
\@namedef{num@ho.quadtent.H2.bestname}{Local polynomial}
\@namedef{num@ho.quadtent.H2.vsbest}{1.1}
\@namedef{num@ho.quadtent.H2.vsexact}{0.54}
\@namedef{num@ho.skewtent.1000.best.mse}{2.6\times10^{-9}}
\@namedef{num@ho.skewtent.1000.best.msename}{Local polynomial}
\@namedef{num@ho.skewtent.1000.best.un}{1.3\times10^{-2}}
\@namedef{num@ho.skewtent.1000.best.unname}{S-map}
\@namedef{num@ho.skewtent.1000.cs.mse}{1.1\times10^{-11}}
\@namedef{num@ho.skewtent.1000.cs.splats}{193}
\@namedef{num@ho.skewtent.1000.cs.un}{3.3\times10^{-3}}
\@namedef{num@ho.skewtent.1000.exact.mse}{1.5\times10^{-15}}
\@namedef{num@ho.skewtent.1000.exact.un}{1.5\times10^{-3}}
\@namedef{num@ho.skewtent.1000.mse.ratio}{0.0043}
\@namedef{num@ho.skewtent.1000.un.ratio}{0.26}
\@namedef{num@ho.skewtent.10000.best.mse}{2.7\times10^{-12}}
\@namedef{num@ho.skewtent.10000.best.msename}{Local polynomial}
\@namedef{num@ho.skewtent.10000.best.un}{2.1\times10^{-3}}
\@namedef{num@ho.skewtent.10000.best.unname}{Local polynomial}
\@namedef{num@ho.skewtent.10000.cs.mse}{1.1\times10^{-13}}
\@namedef{num@ho.skewtent.10000.cs.splats}{301}
\@namedef{num@ho.skewtent.10000.cs.un}{1.5\times10^{-3}}
\@namedef{num@ho.skewtent.10000.exact.mse}{1.5\times10^{-15}}
\@namedef{num@ho.skewtent.10000.exact.un}{1.5\times10^{-3}}
\@namedef{num@ho.skewtent.10000.mse.ratio}{0.041}
\@namedef{num@ho.skewtent.10000.un.ratio}{0.74}
\@namedef{num@ho.skewtent.100000.best.mse}{2.2\times10^{-15}}
\@namedef{num@ho.skewtent.100000.best.msename}{Local polynomial}
\@namedef{num@ho.skewtent.100000.best.un}{2.1\times10^{-3}}
\@namedef{num@ho.skewtent.100000.best.unname}{Local polynomial}
\@namedef{num@ho.skewtent.100000.cs.mse}{1.7\times10^{-15}}
\@namedef{num@ho.skewtent.100000.cs.splats}{338}
\@namedef{num@ho.skewtent.100000.cs.un}{1.5\times10^{-3}}
\@namedef{num@ho.skewtent.100000.exact.mse}{1.5\times10^{-15}}
\@namedef{num@ho.skewtent.100000.exact.un}{1.5\times10^{-3}}
\@namedef{num@ho.skewtent.100000.mse.ratio}{0.77}
\@namedef{num@ho.skewtent.100000.un.ratio}{0.69}
\@namedef{num@ho.skewtent.900000.best.mse}{1.7\times10^{-15}}
\@namedef{num@ho.skewtent.900000.best.msename}{Local polynomial}
\@namedef{num@ho.skewtent.900000.best.un}{1.6\times10^{-3}}
\@namedef{num@ho.skewtent.900000.best.unname}{S-map}
\@namedef{num@ho.skewtent.900000.cs.mse}{1.2\times10^{-15}}
\@namedef{num@ho.skewtent.900000.cs.splats}{670}
\@namedef{num@ho.skewtent.900000.cs.un}{1.3\times10^{-3}}
\@namedef{num@ho.skewtent.900000.exact.mse}{1.5\times10^{-15}}
\@namedef{num@ho.skewtent.900000.exact.un}{1.5\times10^{-3}}
\@namedef{num@ho.skewtent.900000.mse.ratio}{0.73}
\@namedef{num@ho.skewtent.900000.un.ratio}{0.79}
\@namedef{num@ho.skewtent.H2.bestname}{Local polynomial}
\@namedef{num@ho.skewtent.H2.vsbest}{0.73}
\@namedef{num@ho.skewtent.H2.vsexact}{0.82}
\@namedef{num@ho.skewtent.Kexp}{0.18}
\@namedef{num@ho2.H1.cells}{6}
\@namedef{num@ho2.H1.lossmax}{6.4}
\@namedef{num@ho2.H1.lossmin}{1.4}
\@namedef{num@ho2.H1.verdict}{holds}
\@namedef{num@ho2.H1.wins}{4}
\@namedef{num@ho2.H2.verdict}{holds}
\@namedef{num@ho2.H3.max}{5\times10^{11}}
\@namedef{num@ho2.H3.min}{3\times10^{9}}
\@namedef{num@ho2.H3.verdict}{holds}
\@namedef{num@kd.bcnf.far.cs}{4.3\times10^{-16}}
\@namedef{num@kd.bcnf.far.ratio}{1\times10^{5}}
\@namedef{num@kd.bcnf.near5.cs}{100}
\@namedef{num@kd.lozi.far.cs}{1.4\times10^{-15}}
\@namedef{num@kd.lozi.far.ratio}{1\times10^{5}}
\@namedef{num@kd.lozi.near5.cs}{98}
\@namedef{num@kink.bestfloor.max}{33}
\@namedef{num@kink.bestfloor.min}{9.7}
\@namedef{num@kink.globalfloor.min}{3\times10^{7}}
\@namedef{num@kink.ratiofloor.max}{95}
\@namedef{num@kink.ratiofloor.min}{10}
\@namedef{num@kink.ratioglobal.max}{2\times10^{7}}
\@namedef{num@kink.ratioglobal.min}{2\times10^{6}}
\@namedef{num@kink.ratiovb.max}{5\times10^{9}}
\@namedef{num@kink.ratiovb.min}{2\times10^{8}}
\@namedef{num@l63.10000.ChaosSplat}{14.60}
\@namedef{num@l63.10000.ESN}{15.06}
\@namedef{num@l63.10000.ESNclosedloopselection}{15.06}
\@namedef{num@l63.10000.NGRC}{14.60}
\@namedef{num@l63.10000.NGRCclosedloopChaosSplatgrid}{14.60}
\@namedef{num@l63.10000.NGRCclosedloopselection}{15.35}
\@namedef{num@l63.10000.exactmap}{13.65}
\@namedef{num@l63.10000.globalpolynomial}{13.26}
\@namedef{num@l63.2000.ChaosSplat}{14.46}
\@namedef{num@l63.2000.ESN}{14.39}
\@namedef{num@l63.2000.ESNclosedloopselection}{14.39}
\@namedef{num@l63.2000.NGRC}{14.46}
\@namedef{num@l63.2000.NGRCclosedloopChaosSplatgrid}{14.46}
\@namedef{num@l63.2000.NGRCclosedloopselection}{14.46}
\@namedef{num@l63.2000.exactmap}{13.65}
\@namedef{num@l63.2000.globalpolynomial}{13.51}
\@namedef{num@l63.400.ChaosSplat}{11.85}
\@namedef{num@l63.400.ESN}{10.10}
\@namedef{num@l63.400.ESNclosedloopselection}{10.10}
\@namedef{num@l63.400.NGRC}{11.17}
\@namedef{num@l63.400.NGRCclosedloopChaosSplatgrid}{11.85}
\@namedef{num@l63.400.NGRCclosedloopselection}{11.17}
\@namedef{num@l63.400.exactmap}{13.65}
\@namedef{num@l63.400.globalpolynomial}{11.85}
\@namedef{num@l63.ngrc.k.10000}{8}
\@namedef{num@l96.10.ChaosSplat}{13.31}
\@namedef{num@l96.10.ChaosSplatstencil}{13.05}
\@namedef{num@l96.10.ESN}{0.21}
\@namedef{num@l96.10.ESNclosedloopselection}{0.08}
\@namedef{num@l96.10.NGRC}{5.68}
\@namedef{num@l96.10.NGRCclosedloopChaosSplatgrid}{13.31}
\@namedef{num@l96.10.NGRCclosedloopselection}{13.40}
\@namedef{num@l96.10.exactmap}{14.81}
\@namedef{num@l96.10.globalpolynomial}{11.60}
\@namedef{num@l96.10.polynomialstencil}{12.73}
\@namedef{num@l96.20.ChaosSplat}{7.57}
\@namedef{num@l96.20.ChaosSplatstencil}{7.95}
\@namedef{num@l96.20.ESN}{0.23}
\@namedef{num@l96.20.ESNclosedloopselection}{0.10}
\@namedef{num@l96.20.NGRC}{0.12}
\@namedef{num@l96.20.NGRCclosedloopChaosSplatgrid}{7.57}
\@namedef{num@l96.20.NGRCclosedloopselection}{7.57}
\@namedef{num@l96.20.exactmap}{13.11}
\@namedef{num@l96.20.globalpolynomial}{3.94}
\@namedef{num@l96.20.polynomialstencil}{7.72}
\@namedef{num@l96.40.ChaosSplat}{3.72}
\@namedef{num@l96.40.ChaosSplatstencil}{8.01}
\@namedef{num@l96.40.ESN}{0.22}
\@namedef{num@l96.40.ESNclosedloopselection}{0.08}
\@namedef{num@l96.40.NGRC}{0.10}
\@namedef{num@l96.40.NGRCclosedloopChaosSplatgrid}{3.72}
\@namedef{num@l96.40.NGRCclosedloopselection}{3.19}
\@namedef{num@l96.40.exactmap}{12.87}
\@namedef{num@l96.40.globalpolynomial}{0.78}
\@namedef{num@l96.40.polynomialstencil}{7.94}
\@namedef{num@l96.5.ChaosSplat}{13.96}
\@namedef{num@l96.5.ESN}{13.07}
\@namedef{num@l96.5.ESNclosedloopselection}{13.07}
\@namedef{num@l96.5.NGRC}{14.82}
\@namedef{num@l96.5.NGRCclosedloopChaosSplatgrid}{13.96}
\@namedef{num@l96.5.NGRCclosedloopselection}{14.82}
\@namedef{num@l96.5.exactmap}{14.69}
\@namedef{num@l96.5.globalpolynomial}{12.86}
\@namedef{num@lc.1.1000.ChaosSplat.mse}{2.0\times10^{-16}}
\@namedef{num@lc.1.1000.ChaosSplat.un}{1.9\times10^{-14}}
\@namedef{num@lc.1.1000.ESN.mse}{2.3\times10^{-16}}
\@namedef{num@lc.1.1000.ESN.un}{8.3\times10^{-15}}
\@namedef{num@lc.1.1000.NGRC.mse}{2.2\times10^{-16}}
\@namedef{num@lc.1.1000.NGRC.un}{4.7\times10^{-15}}
\@namedef{num@lc.1.1000.Smap.mse}{1.0\times10^{-15}}
\@namedef{num@lc.1.1000.Smap.un}{2.6\times10^{-4}}
\@namedef{num@lc.1.1000.exactmap.mse}{1.5\times10^{-15}}
\@namedef{num@lc.1.1000.exactmap.un}{5.4\times10^{-12}}
\@namedef{num@lc.1.1000.globalpolynomial.mse}{2.0\times10^{-16}}
\@namedef{num@lc.1.1000.globalpolynomial.un}{1.9\times10^{-14}}
\@namedef{num@lc.1.1000.localpolynomial.mse}{2.0\times10^{-16}}
\@namedef{num@lc.1.1000.localpolynomial.un}{1.9\times10^{-14}}
\@namedef{num@lc.1.10000.ChaosSplat.mse}{1.4\times10^{-16}}
\@namedef{num@lc.1.10000.ChaosSplat.un}{3.0\times10^{-15}}
\@namedef{num@lc.1.10000.ESN.mse}{1.7\times10^{-16}}
\@namedef{num@lc.1.10000.ESN.un}{4.1\times10^{-15}}
\@namedef{num@lc.1.10000.NGRC.mse}{1.6\times10^{-16}}
\@namedef{num@lc.1.10000.NGRC.un}{2.9\times10^{-15}}
\@namedef{num@lc.1.10000.RBFnetwork.mse}{1.5\times10^{-16}}
\@namedef{num@lc.1.10000.RBFnetwork.un}{2.8\times10^{-15}}
\@namedef{num@lc.1.10000.Smap.mse}{3.5\times10^{-16}}
\@namedef{num@lc.1.10000.Smap.un}{9.7\times10^{-15}}
\@namedef{num@lc.1.10000.exactmap.mse}{1.5\times10^{-15}}
\@namedef{num@lc.1.10000.exactmap.un}{5.4\times10^{-12}}
\@namedef{num@lc.1.10000.globalpolynomial.mse}{1.4\times10^{-16}}
\@namedef{num@lc.1.10000.globalpolynomial.un}{3.0\times10^{-15}}
\@namedef{num@lc.1.10000.localpolynomial.mse}{1.4\times10^{-16}}
\@namedef{num@lc.1.10000.localpolynomial.un}{2.7\times10^{-15}}
\@namedef{num@lc.1.100000.ChaosSplat.mse}{8.7\times10^{-17}}
\@namedef{num@lc.1.100000.ChaosSplat.un}{1.4\times10^{-15}}
\@namedef{num@lc.1.100000.ESN.mse}{1.3\times10^{-16}}
\@namedef{num@lc.1.100000.ESN.un}{5.6\times10^{-15}}
\@namedef{num@lc.1.100000.NGRC.mse}{1.9\times10^{-16}}
\@namedef{num@lc.1.100000.NGRC.un}{9.9\times10^{-15}}
\@namedef{num@lc.1.100000.RBFnetwork.mse}{1.8\times10^{-16}}
\@namedef{num@lc.1.100000.RBFnetwork.un}{2.8\times10^{-15}}
\@namedef{num@lc.1.100000.Smap.mse}{2.2\times10^{-16}}
\@namedef{num@lc.1.100000.Smap.un}{3.6\times10^{-14}}
\@namedef{num@lc.1.100000.exactmap.mse}{1.5\times10^{-15}}
\@namedef{num@lc.1.100000.exactmap.un}{5.4\times10^{-12}}
\@namedef{num@lc.1.100000.globalpolynomial.mse}{1.5\times10^{-16}}
\@namedef{num@lc.1.100000.globalpolynomial.un}{5.8\times10^{-15}}
\@namedef{num@lc.1.100000.localpolynomial.mse}{8.3\times10^{-17}}
\@namedef{num@lc.1.100000.localpolynomial.un}{1.4\times10^{-15}}
\@namedef{num@lc.2.1000.ChaosSplat.mse}{6.3\times10^{-16}}
\@namedef{num@lc.2.1000.ChaosSplat.un}{2.8\times10^{-7}}
\@namedef{num@lc.2.1000.ESN.mse}{7.6\times10^{-16}}
\@namedef{num@lc.2.1000.ESN.un}{3.7\times10^{-7}}
\@namedef{num@lc.2.1000.NGRC.mse}{1.0\times10^{-15}}
\@namedef{num@lc.2.1000.NGRC.un}{8.7\times10^{-7}}
\@namedef{num@lc.2.1000.Smap.mse}{3.7\times10^{-13}}
\@namedef{num@lc.2.1000.Smap.un}{1.1\times10^{3}}
\@namedef{num@lc.2.1000.exactmap.mse}{1.6\times10^{-15}}
\@namedef{num@lc.2.1000.exactmap.un}{1.5\times10^{-6}}
\@namedef{num@lc.2.1000.globalpolynomial.mse}{6.3\times10^{-16}}
\@namedef{num@lc.2.1000.globalpolynomial.un}{2.8\times10^{-7}}
\@namedef{num@lc.2.1000.localpolynomial.mse}{6.5\times10^{-16}}
\@namedef{num@lc.2.1000.localpolynomial.un}{3.1\times10^{-7}}
\@namedef{num@lc.2.10000.ChaosSplat.mse}{5.4\times10^{-16}}
\@namedef{num@lc.2.10000.ChaosSplat.un}{2.1\times10^{-7}}
\@namedef{num@lc.2.10000.ESN.mse}{6.4\times10^{-16}}
\@namedef{num@lc.2.10000.ESN.un}{3.0\times10^{-7}}
\@namedef{num@lc.2.10000.NGRC.mse}{9.5\times10^{-16}}
\@namedef{num@lc.2.10000.NGRC.un}{7.9\times10^{-7}}
\@namedef{num@lc.2.10000.RBFnetwork.mse}{7.6\times10^{-16}}
\@namedef{num@lc.2.10000.RBFnetwork.un}{3.7\times10^{-7}}
\@namedef{num@lc.2.10000.Smap.mse}{1.7\times10^{-14}}
\@namedef{num@lc.2.10000.Smap.un}{1.4}
\@namedef{num@lc.2.10000.exactmap.mse}{1.6\times10^{-15}}
\@namedef{num@lc.2.10000.exactmap.un}{1.5\times10^{-6}}
\@namedef{num@lc.2.10000.globalpolynomial.mse}{5.4\times10^{-16}}
\@namedef{num@lc.2.10000.globalpolynomial.un}{2.1\times10^{-7}}
\@namedef{num@lc.2.10000.localpolynomial.mse}{5.5\times10^{-16}}
\@namedef{num@lc.2.10000.localpolynomial.un}{2.1\times10^{-7}}
\@namedef{num@lc.2.100000.ChaosSplat.mse}{5.2\times10^{-16}}
\@namedef{num@lc.2.100000.ChaosSplat.un}{1.8\times10^{-7}}
\@namedef{num@lc.2.100000.ESN.mse}{6.5\times10^{-16}}
\@namedef{num@lc.2.100000.ESN.un}{2.9\times10^{-7}}
\@namedef{num@lc.2.100000.NGRC.mse}{9.5\times10^{-16}}
\@namedef{num@lc.2.100000.NGRC.un}{8.1\times10^{-7}}
\@namedef{num@lc.2.100000.RBFnetwork.mse}{9.0\times10^{-16}}
\@namedef{num@lc.2.100000.RBFnetwork.un}{4.6\times10^{-7}}
\@namedef{num@lc.2.100000.Smap.mse}{6.4\times10^{-15}}
\@namedef{num@lc.2.100000.Smap.un}{1.0\times10^{-1}}
\@namedef{num@lc.2.100000.exactmap.mse}{1.6\times10^{-15}}
\@namedef{num@lc.2.100000.exactmap.un}{1.5\times10^{-6}}
\@namedef{num@lc.2.100000.globalpolynomial.mse}{5.0\times10^{-16}}
\@namedef{num@lc.2.100000.globalpolynomial.un}{1.9\times10^{-7}}
\@namedef{num@lc.2.100000.localpolynomial.mse}{4.9\times10^{-16}}
\@namedef{num@lc.2.100000.localpolynomial.un}{1.7\times10^{-7}}
\@namedef{num@lc.3.1000.ChaosSplat.mse}{5.9\times10^{-16}}
\@namedef{num@lc.3.1000.ChaosSplat.un}{1.1\times10^{-3}}
\@namedef{num@lc.3.1000.ESN.mse}{8.2\times10^{-16}}
\@namedef{num@lc.3.1000.ESN.un}{2.7\times10^{8}}
\@namedef{num@lc.3.1000.NGRC.mse}{1.0\times10^{-15}}
\@namedef{num@lc.3.1000.NGRC.un}{2.7\times10^{8}}
\@namedef{num@lc.3.1000.Smap.mse}{4.4\times10^{-13}}
\@namedef{num@lc.3.1000.Smap.un}{5.8\times10^{11}}
\@namedef{num@lc.3.1000.exactmap.mse}{1.5\times10^{-15}}
\@namedef{num@lc.3.1000.exactmap.un}{6.7\times10^{-3}}
\@namedef{num@lc.3.1000.globalpolynomial.mse}{5.9\times10^{-16}}
\@namedef{num@lc.3.1000.globalpolynomial.un}{1.1\times10^{-3}}
\@namedef{num@lc.3.1000.localpolynomial.mse}{6.2\times10^{-16}}
\@namedef{num@lc.3.1000.localpolynomial.un}{1.8\times10^{-3}}
\@namedef{num@lc.3.10000.ChaosSplat.mse}{4.5\times10^{-16}}
\@namedef{num@lc.3.10000.ChaosSplat.un}{2.7\times10^{-4}}
\@namedef{num@lc.3.10000.ESN.mse}{6.7\times10^{-16}}
\@namedef{num@lc.3.10000.ESN.un}{2.7\times10^{8}}
\@namedef{num@lc.3.10000.NGRC.mse}{1.0\times10^{-15}}
\@namedef{num@lc.3.10000.NGRC.un}{5.9\times10^{-3}}
\@namedef{num@lc.3.10000.RBFnetwork.mse}{6.4\times10^{-16}}
\@namedef{num@lc.3.10000.RBFnetwork.un}{7.6\times10^{-4}}
\@namedef{num@lc.3.10000.Smap.mse}{3.1\times10^{-14}}
\@namedef{num@lc.3.10000.Smap.un}{2.7\times10^{4}}
\@namedef{num@lc.3.10000.exactmap.mse}{1.5\times10^{-15}}
\@namedef{num@lc.3.10000.exactmap.un}{6.7\times10^{-3}}
\@namedef{num@lc.3.10000.globalpolynomial.mse}{4.5\times10^{-16}}
\@namedef{num@lc.3.10000.globalpolynomial.un}{2.7\times10^{-4}}
\@namedef{num@lc.3.10000.localpolynomial.mse}{4.8\times10^{-16}}
\@namedef{num@lc.3.10000.localpolynomial.un}{1.1\times10^{-3}}
\@namedef{num@lc.3.100000.ChaosSplat.mse}{4.3\times10^{-16}}
\@namedef{num@lc.3.100000.ChaosSplat.un}{3.1\times10^{-4}}
\@namedef{num@lc.3.100000.ESN.mse}{8.5\times10^{-16}}
\@namedef{num@lc.3.100000.ESN.un}{1.5\times10^{6}}
\@namedef{num@lc.3.100000.NGRC.mse}{1.0\times10^{-15}}
\@namedef{num@lc.3.100000.NGRC.un}{5.8\times10^{-3}}
\@namedef{num@lc.3.100000.RBFnetwork.mse}{6.9\times10^{-16}}
\@namedef{num@lc.3.100000.RBFnetwork.un}{1.6\times10^{-3}}
\@namedef{num@lc.3.100000.Smap.mse}{4.8\times10^{-15}}
\@namedef{num@lc.3.100000.Smap.un}{5.9\times10^{-3}}
\@namedef{num@lc.3.100000.exactmap.mse}{1.5\times10^{-15}}
\@namedef{num@lc.3.100000.exactmap.un}{6.7\times10^{-3}}
\@namedef{num@lc.3.100000.globalpolynomial.mse}{4.3\times10^{-16}}
\@namedef{num@lc.3.100000.globalpolynomial.un}{3.1\times10^{-4}}
\@namedef{num@lc.3.100000.localpolynomial.mse}{4.3\times10^{-16}}
\@namedef{num@lc.3.100000.localpolynomial.un}{2.0\times10^{-4}}
\@namedef{num@lc.4.1000.ChaosSplat.mse}{1.8\times10^{-8}}
\@namedef{num@lc.4.1000.ChaosSplat.un}{1.8\times10^{-1}}
\@namedef{num@lc.4.1000.ESN.mse}{1.1\times10^{-7}}
\@namedef{num@lc.4.1000.ESN.un}{9.8\times10^{-1}}
\@namedef{num@lc.4.1000.NGRC.mse}{2.0\times10^{-3}}
\@namedef{num@lc.4.1000.NGRC.un}{5.6\times10^{12}}
\@namedef{num@lc.4.1000.Smap.mse}{4.0\times10^{-8}}
\@namedef{num@lc.4.1000.Smap.un}{6.8\times10^{-1}}
\@namedef{num@lc.4.1000.exactmap.mse}{2.5\times10^{-15}}
\@namedef{num@lc.4.1000.exactmap.un}{1.1\times10^{-1}}
\@namedef{num@lc.4.1000.globalpolynomial.mse}{1.2\times10^{-4}}
\@namedef{num@lc.4.1000.globalpolynomial.un}{1.5\times10^{11}}
\@namedef{num@lc.4.1000.localpolynomial.mse}{3.3\times10^{-8}}
\@namedef{num@lc.4.1000.localpolynomial.un}{5.8\times10^{-1}}
\@namedef{num@lc.4.10000.ChaosSplat.mse}{4.5\times10^{-11}}
\@namedef{num@lc.4.10000.ChaosSplat.un}{1.9\times10^{-1}}
\@namedef{num@lc.4.10000.ESN.mse}{1.8\times10^{-8}}
\@namedef{num@lc.4.10000.ESN.un}{2.8\times10^{9}}
\@namedef{num@lc.4.10000.NGRC.mse}{1.9\times10^{-3}}
\@namedef{num@lc.4.10000.NGRC.un}{5.6\times10^{12}}
\@namedef{num@lc.4.10000.RBFnetwork.mse}{5.3\times10^{-12}}
\@namedef{num@lc.4.10000.RBFnetwork.un}{2.8\times10^{-1}}
\@namedef{num@lc.4.10000.Smap.mse}{4.4\times10^{-14}}
\@namedef{num@lc.4.10000.Smap.un}{2.5\times10^{-1}}
\@namedef{num@lc.4.10000.exactmap.mse}{2.5\times10^{-15}}
\@namedef{num@lc.4.10000.exactmap.un}{1.1\times10^{-1}}
\@namedef{num@lc.4.10000.globalpolynomial.mse}{1.2\times10^{-4}}
\@namedef{num@lc.4.10000.globalpolynomial.un}{1.6\times10^{11}}
\@namedef{num@lc.4.10000.localpolynomial.mse}{1.5\times10^{-10}}
\@namedef{num@lc.4.10000.localpolynomial.un}{3.0\times10^{-1}}
\@namedef{num@lc.4.100000.ChaosSplat.mse}{3.0\times10^{-15}}
\@namedef{num@lc.4.100000.ChaosSplat.un}{1.1\times10^{-1}}
\@namedef{num@lc.4.100000.ESN.mse}{1.9\times10^{-8}}
\@namedef{num@lc.4.100000.ESN.un}{1.6\times10^{11}}
\@namedef{num@lc.4.100000.NGRC.mse}{1.9\times10^{-3}}
\@namedef{num@lc.4.100000.NGRC.un}{5.6\times10^{12}}
\@namedef{num@lc.4.100000.RBFnetwork.mse}{8.2\times10^{-12}}
\@namedef{num@lc.4.100000.RBFnetwork.un}{2.6\times10^{-1}}
\@namedef{num@lc.4.100000.Smap.mse}{4.7\times10^{-15}}
\@namedef{num@lc.4.100000.Smap.un}{1.4\times10^{-1}}
\@namedef{num@lc.4.100000.exactmap.mse}{2.5\times10^{-15}}
\@namedef{num@lc.4.100000.exactmap.un}{1.1\times10^{-1}}
\@namedef{num@lc.4.100000.globalpolynomial.mse}{1.2\times10^{-4}}
\@namedef{num@lc.4.100000.globalpolynomial.un}{1.7\times10^{11}}
\@namedef{num@lc.4.100000.localpolynomial.mse}{3.1\times10^{-15}}
\@namedef{num@lc.4.100000.localpolynomial.un}{1.2\times10^{-1}}
\@namedef{num@lc.5.1000.ChaosSplat.mse}{3.2\times10^{-7}}
\@namedef{num@lc.5.1000.ChaosSplat.un}{5.1\times10^{-1}}
\@namedef{num@lc.5.1000.ESN.mse}{4.5\times10^{-6}}
\@namedef{num@lc.5.1000.ESN.un}{2.5\times10^{11}}
\@namedef{num@lc.5.1000.NGRC.mse}{2.1\times10^{-2}}
\@namedef{num@lc.5.1000.NGRC.un}{1.7}
\@namedef{num@lc.5.1000.Smap.mse}{1.6\times10^{-9}}
\@namedef{num@lc.5.1000.Smap.un}{9.6\times10^{-1}}
\@namedef{num@lc.5.1000.exactmap.mse}{4.0\times10^{-15}}
\@namedef{num@lc.5.1000.exactmap.un}{4.4\times10^{-1}}
\@namedef{num@lc.5.1000.globalpolynomial.mse}{8.3\times10^{-4}}
\@namedef{num@lc.5.1000.globalpolynomial.un}{5.1\times10^{12}}
\@namedef{num@lc.5.1000.localpolynomial.mse}{2.4\times10^{-9}}
\@namedef{num@lc.5.1000.localpolynomial.un}{1.0}
\@namedef{num@lc.5.10000.ChaosSplat.mse}{4.0\times10^{-15}}
\@namedef{num@lc.5.10000.ChaosSplat.un}{4.4\times10^{-1}}
\@namedef{num@lc.5.10000.ESN.mse}{7.0\times10^{-7}}
\@namedef{num@lc.5.10000.ESN.un}{6.2\times10^{12}}
\@namedef{num@lc.5.10000.NGRC.mse}{2.0\times10^{-2}}
\@namedef{num@lc.5.10000.NGRC.un}{2.4\times10^{9}}
\@namedef{num@lc.5.10000.RBFnetwork.mse}{1.4\times10^{-10}}
\@namedef{num@lc.5.10000.RBFnetwork.un}{7.0\times10^{-1}}
\@namedef{num@lc.5.10000.Smap.mse}{2.3\times10^{-11}}
\@namedef{num@lc.5.10000.Smap.un}{5.7\times10^{-1}}
\@namedef{num@lc.5.10000.exactmap.mse}{4.0\times10^{-15}}
\@namedef{num@lc.5.10000.exactmap.un}{4.4\times10^{-1}}
\@namedef{num@lc.5.10000.globalpolynomial.mse}{8.2\times10^{-4}}
\@namedef{num@lc.5.10000.globalpolynomial.un}{5.1\times10^{12}}
\@namedef{num@lc.5.10000.localpolynomial.mse}{5.8\times10^{-11}}
\@namedef{num@lc.5.10000.localpolynomial.un}{4.6\times10^{-1}}
\@namedef{num@lc.5.100000.ChaosSplat.mse}{4.1\times10^{-15}}
\@namedef{num@lc.5.100000.ChaosSplat.un}{4.3\times10^{-1}}
\@namedef{num@lc.5.100000.ESN.mse}{8.7\times10^{-7}}
\@namedef{num@lc.5.100000.ESN.un}{2.6\times10^{12}}
\@namedef{num@lc.5.100000.NGRC.mse}{2.0\times10^{-2}}
\@namedef{num@lc.5.100000.NGRC.un}{1.8}
\@namedef{num@lc.5.100000.RBFnetwork.mse}{1.5\times10^{-10}}
\@namedef{num@lc.5.100000.RBFnetwork.un}{6.5\times10^{-1}}
\@namedef{num@lc.5.100000.Smap.mse}{4.9\times10^{-15}}
\@namedef{num@lc.5.100000.Smap.un}{4.5\times10^{-1}}
\@namedef{num@lc.5.100000.exactmap.mse}{4.0\times10^{-15}}
\@namedef{num@lc.5.100000.exactmap.un}{4.4\times10^{-1}}
\@namedef{num@lc.5.100000.globalpolynomial.mse}{8.2\times10^{-4}}
\@namedef{num@lc.5.100000.globalpolynomial.un}{5.1\times10^{12}}
\@namedef{num@lc.5.100000.localpolynomial.mse}{4.8\times10^{-15}}
\@namedef{num@lc.5.100000.localpolynomial.un}{4.5\times10^{-1}}
\@namedef{num@lc.6.1000.ChaosSplat.mse}{3.2\times10^{-8}}
\@namedef{num@lc.6.1000.ChaosSplat.un}{7.1\times10^{-1}}
\@namedef{num@lc.6.1000.ESN.mse}{1.3\times10^{-5}}
\@namedef{num@lc.6.1000.ESN.un}{3.9\times10^{10}}
\@namedef{num@lc.6.1000.NGRC.mse}{7.2\times10^{-2}}
\@namedef{num@lc.6.1000.NGRC.un}{1.3}
\@namedef{num@lc.6.1000.Smap.mse}{4.2\times10^{-9}}
\@namedef{num@lc.6.1000.Smap.un}{1.1}
\@namedef{num@lc.6.1000.exactmap.mse}{5.7\times10^{-15}}
\@namedef{num@lc.6.1000.exactmap.un}{7.0\times10^{-1}}
\@namedef{num@lc.6.1000.globalpolynomial.mse}{3.1\times10^{-3}}
\@namedef{num@lc.6.1000.globalpolynomial.un}{4.8\times10^{12}}
\@namedef{num@lc.6.1000.localpolynomial.mse}{1.2\times10^{-7}}
\@namedef{num@lc.6.1000.localpolynomial.un}{7.4\times10^{-1}}
\@namedef{num@lc.6.10000.ChaosSplat.mse}{3.4\times10^{-11}}
\@namedef{num@lc.6.10000.ChaosSplat.un}{7.1\times10^{-1}}
\@namedef{num@lc.6.10000.ESN.mse}{1.6\times10^{-6}}
\@namedef{num@lc.6.10000.ESN.un}{6.4\times10^{12}}
\@namedef{num@lc.6.10000.NGRC.mse}{7.1\times10^{-2}}
\@namedef{num@lc.6.10000.NGRC.un}{1.3}
\@namedef{num@lc.6.10000.RBFnetwork.mse}{1.1\times10^{-10}}
\@namedef{num@lc.6.10000.RBFnetwork.un}{8.4\times10^{-1}}
\@namedef{num@lc.6.10000.Smap.mse}{1.8\times10^{-12}}
\@namedef{num@lc.6.10000.Smap.un}{8.4\times10^{-1}}
\@namedef{num@lc.6.10000.exactmap.mse}{5.7\times10^{-15}}
\@namedef{num@lc.6.10000.exactmap.un}{7.0\times10^{-1}}
\@namedef{num@lc.6.10000.globalpolynomial.mse}{3.1\times10^{-3}}
\@namedef{num@lc.6.10000.globalpolynomial.un}{5.0\times10^{12}}
\@namedef{num@lc.6.10000.localpolynomial.mse}{6.9\times10^{-12}}
\@namedef{num@lc.6.10000.localpolynomial.un}{7.4\times10^{-1}}
\@namedef{num@lc.6.100000.ChaosSplat.mse}{5.8\times10^{-15}}
\@namedef{num@lc.6.100000.ChaosSplat.un}{7.0\times10^{-1}}
\@namedef{num@lc.6.100000.ESN.mse}{2.3\times10^{-6}}
\@namedef{num@lc.6.100000.ESN.un}{5.2\times10^{12}}
\@namedef{num@lc.6.100000.NGRC.mse}{7.0\times10^{-2}}
\@namedef{num@lc.6.100000.NGRC.un}{1.3}
\@namedef{num@lc.6.100000.RBFnetwork.mse}{1.2\times10^{-10}}
\@namedef{num@lc.6.100000.RBFnetwork.un}{9.8\times10^{-1}}
\@namedef{num@lc.6.100000.Smap.mse}{6.8\times10^{-15}}
\@namedef{num@lc.6.100000.Smap.un}{7.1\times10^{-1}}
\@namedef{num@lc.6.100000.exactmap.mse}{5.7\times10^{-15}}
\@namedef{num@lc.6.100000.exactmap.un}{7.0\times10^{-1}}
\@namedef{num@lc.6.100000.globalpolynomial.mse}{3.1\times10^{-3}}
\@namedef{num@lc.6.100000.globalpolynomial.un}{5.0\times10^{12}}
\@namedef{num@lc.6.100000.localpolynomial.mse}{6.8\times10^{-15}}
\@namedef{num@lc.6.100000.localpolynomial.un}{7.0\times10^{-1}}
\@namedef{num@lc.smooth.floor.max}{3.8}
\@namedef{num@lor.ar.mse}{1.8\times10^{-10}}
\@namedef{num@lor.ar.un}{5.9\times10^{-3}}
\@namedef{num@lor.best.mse}{5.9\times10^{-14}}
\@namedef{num@lor.best.name}{Local polynomial, own window}
\@namedef{num@lor.best20.name}{Local polynomial, own window}
\@namedef{num@lor.best20.un}{1.2\times10^{-14}}
\@namedef{num@lor.cs.m}{14}
\@namedef{num@lor.cs.mse}{9.7\times10^{-14}}
\@namedef{num@lor.cs.size}{2.5\times10^{4}}
\@namedef{num@lor.cs.splats}{181}
\@namedef{num@lor.cs.un}{3.3\times10^{-12}}
\@namedef{num@lor.esn.m}{100}
\@namedef{num@lor.esn.mse}{1.5\times10^{-13}}
\@namedef{num@lor.esn.un}{1.3\times10^{-11}}
\@namedef{num@lor.lp.m}{14}
\@namedef{num@lor.lp.mse}{6.2\times10^{-14}}
\@namedef{num@lor.lp.un}{1.5\times10^{-14}}
\@namedef{num@lor.lpo.m}{16}
\@namedef{num@lor.lpo.mse}{5.9\times10^{-14}}
\@namedef{num@lor.lpo.un}{1.2\times10^{-14}}
\@namedef{num@lor.ngrc.m}{16}
\@namedef{num@lor.ngrc.mse}{2.1\times10^{-13}}
\@namedef{num@lor.ngrc.un}{6.2\times10^{-10}}
\@namedef{num@lor.poly.m}{12}
\@namedef{num@lor.poly.mse}{3.2\times10^{-13}}
\@namedef{num@lor.poly.un}{4.7\times10^{-9}}
\@namedef{num@lor.ratio}{0.6}
\@namedef{num@lor.ratio20}{0.0037}
\@namedef{num@lor.ratioglobal}{2}
\@namedef{num@lor.rbf.m}{14}
\@namedef{num@lor.rbf.mse}{1.3\times10^{-12}}
\@namedef{num@lor.rbf.un}{1.5\times10^{-8}}
\@namedef{num@lor.smap.m}{14}
\@namedef{num@lor.smap.mse}{3.0\times10^{-13}}
\@namedef{num@lor.smap.un}{2.7\times10^{-11}}
\@namedef{num@lor.smapo.m}{16}
\@namedef{num@lor.smapo.mse}{3.0\times10^{-13}}
\@namedef{num@lor.smapo.un}{7.6\times10^{-11}}
\@namedef{num@lr.1.cs}{never}
\@namedef{num@lr.1.exact}{never}
\@namedef{num@lr.2.cs}{76}
\@namedef{num@lr.2.exact}{70}
\@namedef{num@lr.3.cs}{52}
\@namedef{num@lr.3.exact}{48}
\@namedef{num@lr.4.cs}{41}
\@namedef{num@lr.4.exact}{39}
\@namedef{num@lr.5.cs}{33}
\@namedef{num@lr.5.exact}{31}
\@namedef{num@lr.6.cs}{27}
\@namedef{num@lr.6.exact}{27}
\@namedef{num@lr.henon.cs}{87}
\@namedef{num@lr.henon.exact}{79}
\@namedef{num@lr.lorenz.cs}{544}
\@namedef{num@lr.rossler.cs}{1{,}022}
\@namedef{num@lr2.1.cs.lost}{never}
\@namedef{num@lr2.1.cs.stepzero}{never}
\@namedef{num@lr2.1.cs.zero}{never}
\@namedef{num@lr2.1.esn.lost}{never}
\@namedef{num@lr2.1.esn.stepzero}{never}
\@namedef{num@lr2.1.esn.zero}{never}
\@namedef{num@lr2.1.lp.lost}{never}
\@namedef{num@lr2.1.lp.stepzero}{never}
\@namedef{num@lr2.1.lp.zero}{never}
\@namedef{num@lr2.1.ngrc.lost}{never}
\@namedef{num@lr2.1.ngrc.stepzero}{never}
\@namedef{num@lr2.1.ngrc.zero}{never}
\@namedef{num@lr2.1.poly.lost}{never}
\@namedef{num@lr2.1.poly.stepzero}{never}
\@namedef{num@lr2.1.poly.zero}{never}
\@namedef{num@lr2.1.ratio.max}{16}
\@namedef{num@lr2.1.smap.lost}{never}
\@namedef{num@lr2.1.smap.stepzero}{never}
\@namedef{num@lr2.1.smap.zero}{never}
\@namedef{num@lr2.1.twice.until}{464}
\@namedef{num@lr2.2.cs.lost}{44}
\@namedef{num@lr2.2.cs.stepzero}{38}
\@namedef{num@lr2.2.cs.zero}{76}
\@namedef{num@lr2.2.esn.lost}{42}
\@namedef{num@lr2.2.esn.stepzero}{37}
\@namedef{num@lr2.2.esn.zero}{73}
\@namedef{num@lr2.2.lp.lost}{44}
\@namedef{num@lr2.2.lp.stepzero}{39}
\@namedef{num@lr2.2.lp.zero}{76}
\@namedef{num@lr2.2.ngrc.lost}{41}
\@namedef{num@lr2.2.ngrc.stepzero}{36}
\@namedef{num@lr2.2.ngrc.zero}{72}
\@namedef{num@lr2.2.poly.lost}{44}
\@namedef{num@lr2.2.poly.stepzero}{38}
\@namedef{num@lr2.2.poly.zero}{76}
\@namedef{num@lr2.2.smap.lost}{43}
\@namedef{num@lr2.2.smap.stepzero}{38}
\@namedef{num@lr2.2.smap.zero}{75}
\@namedef{num@lr2.3.cs.lost}{28}
\@namedef{num@lr2.3.cs.stepzero}{26}
\@namedef{num@lr2.3.cs.zero}{52}
\@namedef{num@lr2.3.esn.lost}{26}
\@namedef{num@lr2.3.esn.stepzero}{25}
\@namedef{num@lr2.3.esn.zero}{48}
\@namedef{num@lr2.3.lp.lost}{28}
\@namedef{num@lr2.3.lp.stepzero}{26}
\@namedef{num@lr2.3.lp.zero}{52}
\@namedef{num@lr2.3.ngrc.lost}{26}
\@namedef{num@lr2.3.ngrc.stepzero}{25}
\@namedef{num@lr2.3.ngrc.zero}{47}
\@namedef{num@lr2.3.poly.lost}{28}
\@namedef{num@lr2.3.poly.stepzero}{26}
\@namedef{num@lr2.3.poly.zero}{51}
\@namedef{num@lr2.3.smap.lost}{27}
\@namedef{num@lr2.3.smap.stepzero}{26}
\@namedef{num@lr2.3.smap.zero}{50}
\@namedef{num@lr2.4.cs.lost}{22}
\@namedef{num@lr2.4.cs.stepzero}{21}
\@namedef{num@lr2.4.cs.zero}{41}
\@namedef{num@lr2.4.esn.lost}{10}
\@namedef{num@lr2.4.esn.stepzero}{9}
\@namedef{num@lr2.4.esn.zero}{9}
\@namedef{num@lr2.4.lp.lost}{23}
\@namedef{num@lr2.4.lp.stepzero}{21}
\@namedef{num@lr2.4.lp.zero}{41}
\@namedef{num@lr2.4.ngrc.lost}{3}
\@namedef{num@lr2.4.ngrc.stepzero}{3}
\@namedef{num@lr2.4.ngrc.zero}{3}
\@namedef{num@lr2.4.poly.lost}{14}
\@namedef{num@lr2.4.poly.stepzero}{12}
\@namedef{num@lr2.4.poly.zero}{23}
\@namedef{num@lr2.4.smap.lost}{23}
\@namedef{num@lr2.4.smap.stepzero}{21}
\@namedef{num@lr2.4.smap.zero}{40}
\@namedef{num@lr2.5.cs.lost}{18}
\@namedef{num@lr2.5.cs.stepzero}{17}
\@namedef{num@lr2.5.cs.zero}{33}
\@namedef{num@lr2.5.esn.lost}{6}
\@namedef{num@lr2.5.esn.stepzero}{5}
\@namedef{num@lr2.5.esn.zero}{5}
\@namedef{num@lr2.5.lp.lost}{19}
\@namedef{num@lr2.5.lp.stepzero}{17}
\@namedef{num@lr2.5.lp.zero}{33}
\@namedef{num@lr2.5.ngrc.lost}{3}
\@namedef{num@lr2.5.ngrc.stepzero}{2}
\@namedef{num@lr2.5.ngrc.zero}{3}
\@namedef{num@lr2.5.poly.lost}{11}
\@namedef{num@lr2.5.poly.stepzero}{10}
\@namedef{num@lr2.5.poly.zero}{18}
\@namedef{num@lr2.5.smap.lost}{18}
\@namedef{num@lr2.5.smap.stepzero}{17}
\@namedef{num@lr2.5.smap.zero}{33}
\@namedef{num@lr2.6.cs.lost}{15}
\@namedef{num@lr2.6.cs.stepzero}{14}
\@namedef{num@lr2.6.cs.zero}{27}
\@namedef{num@lr2.6.esn.lost}{4}
\@namedef{num@lr2.6.esn.stepzero}{3}
\@namedef{num@lr2.6.esn.zero}{3}
\@namedef{num@lr2.6.lp.lost}{15}
\@namedef{num@lr2.6.lp.stepzero}{14}
\@namedef{num@lr2.6.lp.zero}{26}
\@namedef{num@lr2.6.ngrc.lost}{never}
\@namedef{num@lr2.6.ngrc.stepzero}{2}
\@namedef{num@lr2.6.ngrc.zero}{3}
\@namedef{num@lr2.6.poly.lost}{9}
\@namedef{num@lr2.6.poly.stepzero}{8}
\@namedef{num@lr2.6.poly.zero}{15}
\@namedef{num@lr2.6.smap.lost}{15}
\@namedef{num@lr2.6.smap.stepzero}{14}
\@namedef{num@lr2.6.smap.zero}{27}
\@namedef{num@lr2.cslocal.maxgap}{2}
\@namedef{num@lr2.cslp.stepgap}{1}
\@namedef{num@lr2.henon.cs.lost}{51}
\@namedef{num@lr2.henon.cs.stepzero}{44}
\@namedef{num@lr2.henon.cs.zero}{87}
\@namedef{num@lr2.henon.esn.lost}{47}
\@namedef{num@lr2.henon.esn.stepzero}{39}
\@namedef{num@lr2.henon.esn.zero}{79}
\@namedef{num@lr2.henon.lp.lost}{53}
\@namedef{num@lr2.henon.lp.stepzero}{44}
\@namedef{num@lr2.henon.lp.zero}{89}
\@namedef{num@lr2.henon.ngrc.lost}{48}
\@namedef{num@lr2.henon.ngrc.stepzero}{41}
\@namedef{num@lr2.henon.ngrc.zero}{81}
\@namedef{num@lr2.henon.poly.lost}{51}
\@namedef{num@lr2.henon.poly.stepzero}{43}
\@namedef{num@lr2.henon.poly.zero}{87}
\@namedef{num@lr2.henon.smap.lost}{47}
\@namedef{num@lr2.henon.smap.stepzero}{39}
\@namedef{num@lr2.henon.smap.zero}{78}
\@namedef{num@lr2.windows.max}{2{,}998}
\@namedef{num@lr2.windows.min}{1{,}798}
\@namedef{num@m1.best.mse}{2.1\times10^{-16}}
\@namedef{num@m1.best.name}{ESN}
\@namedef{num@m1.best.ratiofloor}{1.2}
\@namedef{num@m1.best20.name}{ESN}
\@namedef{num@m1.best20.un}{7.8\times10^{-15}}
\@namedef{num@m1.cs.m}{16}
\@namedef{num@m1.cs.mse}{1.8\times10^{-16}}
\@namedef{num@m1.cs.size}{3.0\times10^{4}}
\@namedef{num@m1.cs.splats}{171}
\@namedef{num@m1.cs.un}{1.4\times10^{-15}}
\@namedef{num@m1.esn.m}{16}
\@namedef{num@m1.esn.mse}{2.1\times10^{-16}}
\@namedef{num@m1.esn.un}{7.8\times10^{-15}}
\@namedef{num@m1.exact.mse}{1.5\times10^{-15}}
\@namedef{num@m1.exact.un}{5.2\times10^{-12}}
\@namedef{num@m1.floor.mse}{1.7\times10^{-16}}
\@namedef{num@m1.lpo.m}{2}
\@namedef{num@m1.lpo.mse}{2.5\times10^{-16}}
\@namedef{num@m1.lpo.un}{6.0\times10^{-14}}
\@namedef{num@m1.ngrc.m}{16}
\@namedef{num@m1.ngrc.mse}{2.3\times10^{-16}}
\@namedef{num@m1.ngrc.un}{3.9\times10^{-14}}
\@namedef{num@m1.poly.m}{6}
\@namedef{num@m1.poly.mse}{2.2\times10^{-16}}
\@namedef{num@m1.poly.un}{3.3\times10^{-14}}
\@namedef{num@m1.ratio}{1.2}
\@namedef{num@m1.ratio20}{5.4}
\@namedef{num@m1.ratioexact}{0.12}
\@namedef{num@m1.ratiofloor}{1.1}
\@namedef{num@m1.ratioglobal}{1}
\@namedef{num@m1.ratiovb}{1\times10^{8}}
\@namedef{num@m1.smapo.m}{2}
\@namedef{num@m1.smapo.mse}{2.1\times10^{-16}}
\@namedef{num@m1.smapo.un}{5.8\times10^{-14}}
\@namedef{num@m1.vb.mse}{1.9\times10^{-8}}
\@namedef{num@m2.best.mse}{4.3\times10^{-16}}
\@namedef{num@m2.best.name}{Local polynomial, own window}
\@namedef{num@m2.best.ratiofloor}{2.2}
\@namedef{num@m2.best20.name}{Local polynomial, own window}
\@namedef{num@m2.best20.un}{1.6\times10^{-7}}
\@namedef{num@m2.cs.m}{4}
\@namedef{num@m2.cs.mse}{4.3\times10^{-16}}
\@namedef{num@m2.cs.size}{2.2\times10^{3}}
\@namedef{num@m2.cs.splats}{94}
\@namedef{num@m2.cs.un}{1.9\times10^{-7}}
\@namedef{num@m2.esn.m}{5}
\@namedef{num@m2.esn.mse}{7.0\times10^{-16}}
\@namedef{num@m2.esn.un}{5.0\times10^{-7}}
\@namedef{num@m2.exact.mse}{1.5\times10^{-15}}
\@namedef{num@m2.exact.un}{1.4\times10^{-6}}
\@namedef{num@m2.floor.mse}{2.0\times10^{-16}}
\@namedef{num@m2.lp.m}{4}
\@namedef{num@m2.lp.mse}{4.3\times10^{-16}}
\@namedef{num@m2.lp.un}{2.0\times10^{-7}}
\@namedef{num@m2.lpo.m}{7}
\@namedef{num@m2.lpo.mse}{4.3\times10^{-16}}
\@namedef{num@m2.lpo.un}{1.6\times10^{-7}}
\@namedef{num@m2.ngrc.m}{5}
\@namedef{num@m2.ngrc.mse}{7.9\times10^{-16}}
\@namedef{num@m2.ngrc.un}{7.8\times10^{-7}}
\@namedef{num@m2.poly.m}{5}
\@namedef{num@m2.poly.mse}{4.4\times10^{-16}}
\@namedef{num@m2.poly.un}{1.7\times10^{-7}}
\@namedef{num@m2.ratio}{0.98}
\@namedef{num@m2.ratio20}{0.84}
\@namedef{num@m2.ratioexact}{0.29}
\@namedef{num@m2.ratiofloor}{2.2}
\@namedef{num@m2.ratioglobal}{1}
\@namedef{num@m2.ratiovb}{6\times10^{7}}
\@namedef{num@m2.rbf.m}{4}
\@namedef{num@m2.rbf.mse}{7.2\times10^{-16}}
\@namedef{num@m2.rbf.un}{4.2\times10^{-7}}
\@namedef{num@m2.smap.m}{4}
\@namedef{num@m2.smap.mse}{6.1\times10^{-16}}
\@namedef{num@m2.smap.un}{2.5\times10^{-7}}
\@namedef{num@m2.smapo.m}{2}
\@namedef{num@m2.smapo.mse}{5.7\times10^{-16}}
\@namedef{num@m2.smapo.un}{3.2\times10^{-7}}
\@namedef{num@m2.vb.mse}{2.5\times10^{-8}}
\@namedef{num@m3.best.mse}{4.0\times10^{-16}}
\@namedef{num@m3.best.name}{Local polynomial}
\@namedef{num@m3.best.ratiofloor}{2.5}
\@namedef{num@m3.best20.name}{Local polynomial}
\@namedef{num@m3.best20.un}{6.6\times10^{-5}}
\@namedef{num@m3.cs.m}{4}
\@namedef{num@m3.cs.mse}{4.1\times10^{-16}}
\@namedef{num@m3.cs.size}{3.9\times10^{3}}
\@namedef{num@m3.cs.splats}{170}
\@namedef{num@m3.cs.un}{6.8\times10^{-5}}
\@namedef{num@m3.esn.m}{4}
\@namedef{num@m3.esn.mse}{1.4\times10^{-15}}
\@namedef{num@m3.esn.un}{7.9\times10^{-3}}
\@namedef{num@m3.exact.mse}{1.4\times10^{-15}}
\@namedef{num@m3.exact.un}{7.8\times10^{-3}}
\@namedef{num@m3.floor.mse}{1.6\times10^{-16}}
\@namedef{num@m3.lp.m}{4}
\@namedef{num@m3.lp.mse}{4.0\times10^{-16}}
\@namedef{num@m3.lp.un}{6.6\times10^{-5}}
\@namedef{num@m3.lpo.m}{4}
\@namedef{num@m3.lpo.mse}{4.0\times10^{-16}}
\@namedef{num@m3.lpo.un}{6.6\times10^{-5}}
\@namedef{num@m3.ngrc.m}{4}
\@namedef{num@m3.ngrc.mse}{8.8\times10^{-16}}
\@namedef{num@m3.ngrc.un}{6.2\times10^{-3}}
\@namedef{num@m3.poly.m}{5}
\@namedef{num@m3.poly.mse}{4.1\times10^{-16}}
\@namedef{num@m3.poly.un}{5.6\times10^{-4}}
\@namedef{num@m3.ratio}{0.99}
\@namedef{num@m3.ratio20}{0.97}
\@namedef{num@m3.ratioexact}{0.29}
\@namedef{num@m3.ratiofloor}{2.5}
\@namedef{num@m3.ratioglobal}{1}
\@namedef{num@m3.ratiovb}{5\times10^{8}}
\@namedef{num@m3.rbf.m}{4}
\@namedef{num@m3.rbf.mse}{6.2\times10^{-16}}
\@namedef{num@m3.rbf.un}{2.7\times10^{-3}}
\@namedef{num@m3.smap.m}{4}
\@namedef{num@m3.smap.mse}{7.0\times10^{-16}}
\@namedef{num@m3.smap.un}{2.4\times10^{-3}}
\@namedef{num@m3.smapo.m}{2}
\@namedef{num@m3.smapo.mse}{5.6\times10^{-16}}
\@namedef{num@m3.smapo.un}{7.9\times10^{-4}}
\@namedef{num@m3.vb.mse}{2.1\times10^{-7}}
\@namedef{num@m4.best.mse}{1.6\times10^{-15}}
\@namedef{num@m4.best.name}{S-map}
\@namedef{num@m4.best.ratiofloor}{9.7}
\@namedef{num@m4.best20.name}{Local polynomial}
\@namedef{num@m4.best20.un}{5.2\times10^{-2}}
\@namedef{num@m4.cheb.mse}{4.7\times10^{-9}}
\@namedef{num@m4.cheb.un}{8.6\times10^{-1}}
\@namedef{num@m4.cs.m}{2}
\@namedef{num@m4.cs.mse}{1.7\times10^{-15}}
\@namedef{num@m4.cs.size}{5.7\times10^{3}}
\@namedef{num@m4.cs.splats}{638}
\@namedef{num@m4.cs.un}{4.2\times10^{-2}}
\@namedef{num@m4.esn.m}{1}
\@namedef{num@m4.esn.mse}{2.1\times10^{-8}}
\@namedef{num@m4.esn.un}{4.8\times10^{10}}
\@namedef{num@m4.exact.mse}{2.4\times10^{-15}}
\@namedef{num@m4.exact.un}{1.2\times10^{-1}}
\@namedef{num@m4.floor.mse}{1.7\times10^{-16}}
\@namedef{num@m4.lp.m}{2}
\@namedef{num@m4.lp.mse}{2.6\times10^{-15}}
\@namedef{num@m4.lp.un}{5.2\times10^{-2}}
\@namedef{num@m4.lpo.m}{2}
\@namedef{num@m4.lpo.mse}{2.6\times10^{-15}}
\@namedef{num@m4.lpo.un}{5.2\times10^{-2}}
\@namedef{num@m4.ngrc.m}{1}
\@namedef{num@m4.ngrc.mse}{1.9\times10^{-3}}
\@namedef{num@m4.ngrc.un}{6.0\times10^{43}}
\@namedef{num@m4.poly.m}{3}
\@namedef{num@m4.poly.mse}{7.6\times10^{-5}}
\@namedef{num@m4.poly.un}{6.7\times10^{12}}
\@namedef{num@m4.ratio}{0.96}
\@namedef{num@m4.ratio20}{1.2}
\@namedef{num@m4.ratioexact}{0.68}
\@namedef{num@m4.ratiofloor}{10}
\@namedef{num@m4.ratioglobal}{3\times10^{6}}
\@namedef{num@m4.ratiovb}{7\times10^{8}}
\@namedef{num@m4.rbf.m}{2}
\@namedef{num@m4.rbf.mse}{1.7\times10^{-10}}
\@namedef{num@m4.rbf.un}{2.4\times10^{3}}
\@namedef{num@m4.smap.m}{2}
\@namedef{num@m4.smap.mse}{1.6\times10^{-15}}
\@namedef{num@m4.smap.un}{5.5\times10^{-2}}
\@namedef{num@m4.smapo.m}{2}
\@namedef{num@m4.smapo.mse}{1.6\times10^{-15}}
\@namedef{num@m4.smapo.un}{5.5\times10^{-2}}
\@namedef{num@m4.vb.mse}{1.2\times10^{-6}}
\@namedef{num@m5.best.mse}{4.0\times10^{-15}}
\@namedef{num@m5.best.name}{S-map}
\@namedef{num@m5.best.ratiofloor}{21}
\@namedef{num@m5.best20.name}{Local polynomial}
\@namedef{num@m5.best20.un}{3.9\times10^{-1}}
\@namedef{num@m5.cheb.mse}{3.8\times10^{-8}}
\@namedef{num@m5.cheb.un}{1.1}
\@namedef{num@m5.cs.m}{2}
\@namedef{num@m5.cs.mse}{1.8\times10^{-14}}
\@namedef{num@m5.cs.size}{5.0\times10^{3}}
\@namedef{num@m5.cs.splats}{558}
\@namedef{num@m5.cs.un}{3.9\times10^{-1}}
\@namedef{num@m5.esn.m}{1}
\@namedef{num@m5.esn.mse}{1.3\times10^{-6}}
\@namedef{num@m5.esn.un}{6.7\times10^{11}}
\@namedef{num@m5.exact.mse}{3.8\times10^{-15}}
\@namedef{num@m5.exact.un}{4.6\times10^{-1}}
\@namedef{num@m5.floor.mse}{1.9\times10^{-16}}
\@namedef{num@m5.lp.m}{2}
\@namedef{num@m5.lp.mse}{9.2\times10^{-15}}
\@namedef{num@m5.lp.un}{3.9\times10^{-1}}
\@namedef{num@m5.lpo.m}{1}
\@namedef{num@m5.lpo.mse}{7.0\times10^{-15}}
\@namedef{num@m5.lpo.un}{4.6\times10^{-1}}
\@namedef{num@m5.ngrc.m}{1}
\@namedef{num@m5.ngrc.mse}{2.1\times10^{-2}}
\@namedef{num@m5.ngrc.un}{3.2\times10^{35}}
\@namedef{num@m5.poly.m}{3}
\@namedef{num@m5.poly.mse}{7.3\times10^{-4}}
\@namedef{num@m5.poly.un}{7.1\times10^{12}}
\@namedef{num@m5.ratio}{0.22}
\@namedef{num@m5.ratio20}{1}
\@namedef{num@m5.ratioexact}{4.8}
\@namedef{num@m5.ratiofloor}{95}
\@namedef{num@m5.ratioglobal}{2\times10^{6}}
\@namedef{num@m5.ratiovb}{2\times10^{8}}
\@namedef{num@m5.rbf.m}{2}
\@namedef{num@m5.rbf.mse}{4.0\times10^{-9}}
\@namedef{num@m5.rbf.un}{9.6\times10^{-1}}
\@namedef{num@m5.smap.m}{2}
\@namedef{num@m5.smap.mse}{4.0\times10^{-15}}
\@namedef{num@m5.smap.un}{3.9\times10^{-1}}
\@namedef{num@m5.smapo.m}{2}
\@namedef{num@m5.smapo.mse}{4.0\times10^{-15}}
\@namedef{num@m5.smapo.un}{3.9\times10^{-1}}
\@namedef{num@m5.vb.mse}{3.6\times10^{-6}}
\@namedef{num@m6.best.mse}{7.3\times10^{-15}}
\@namedef{num@m6.best.name}{S-map}
\@namedef{num@m6.best.ratiofloor}{39}
\@namedef{num@m6.best20.name}{S-map}
\@namedef{num@m6.best20.un}{7.0\times10^{-1}}
\@namedef{num@m6.cheb.mse}{1.4\times10^{-7}}
\@namedef{num@m6.cheb.un}{1.3}
\@namedef{num@m6.cs.m}{1}
\@namedef{num@m6.cs.mse}{6.1\times10^{-15}}
\@namedef{num@m6.cs.size}{1.9\times10^{3}}
\@namedef{num@m6.cs.splats}{381}
\@namedef{num@m6.cs.un}{7.0\times10^{-1}}
\@namedef{num@m6.esn.m}{1}
\@namedef{num@m6.esn.mse}{2.9\times10^{-6}}
\@namedef{num@m6.esn.un}{2.2\times10^{12}}
\@namedef{num@m6.exact.mse}{5.5\times10^{-15}}
\@namedef{num@m6.exact.un}{7.0\times10^{-1}}
\@namedef{num@m6.floor.mse}{1.9\times10^{-16}}
\@namedef{num@m6.lp.m}{1}
\@namedef{num@m6.lp.mse}{8.5\times10^{-15}}
\@namedef{num@m6.lp.un}{7.1\times10^{-1}}
\@namedef{num@m6.lpo.m}{1}
\@namedef{num@m6.lpo.mse}{8.5\times10^{-15}}
\@namedef{num@m6.lpo.un}{7.1\times10^{-1}}
\@namedef{num@m6.ngrc.m}{1}
\@namedef{num@m6.ngrc.mse}{7.0\times10^{-2}}
\@namedef{num@m6.ngrc.un}{1.3}
\@namedef{num@m6.poly.m}{3}
\@namedef{num@m6.poly.mse}{2.9\times10^{-3}}
\@namedef{num@m6.poly.un}{4.9\times10^{12}}
\@namedef{num@m6.ratio}{1.2}
\@namedef{num@m6.ratio20}{1}
\@namedef{num@m6.ratioexact}{1.1}
\@namedef{num@m6.ratiofloor}{33}
\@namedef{num@m6.ratioglobal}{2\times10^{7}}
\@namedef{num@m6.ratiovb}{5\times10^{9}}
\@namedef{num@m6.rbf.m}{1}
\@namedef{num@m6.rbf.mse}{1.0\times10^{-10}}
\@namedef{num@m6.rbf.un}{9.0\times10^{-1}}
\@namedef{num@m6.smap.m}{1}
\@namedef{num@m6.smap.mse}{7.3\times10^{-15}}
\@namedef{num@m6.smap.un}{7.0\times10^{-1}}
\@namedef{num@m6.smapo.m}{1}
\@namedef{num@m6.smapo.mse}{7.3\times10^{-15}}
\@namedef{num@m6.smapo.un}{7.0\times10^{-1}}
\@namedef{num@m6.vb.mse}{2.9\times10^{-5}}
\@namedef{num@maps.csoverbest.max}{4.6}
\@namedef{num@mv.cells}{22}
\@namedef{num@mv.mse.max}{3\times10^{4}}
\@namedef{num@mv.mse.within}{15}
\@namedef{num@mv.un.max}{33}
\@namedef{num@mv.un.within}{18}
\@namedef{num@mv2.H1.wins}{5}
\@namedef{num@mv2.bentlogistic.1000.mse}{1.9\times10^{-12}}
\@namedef{num@mv2.bentlogistic.1000.un}{1.2\times10^{-2}}
\@namedef{num@mv2.bentlogistic.10000.mse}{4.5\times10^{-14}}
\@namedef{num@mv2.bentlogistic.10000.un}{1.1\times10^{-2}}
\@namedef{num@mv2.cells}{6}
\@namedef{num@mv2.curvedtent.1000.mse}{1.6\times10^{-9}}
\@namedef{num@mv2.curvedtent.1000.un}{1.4\times10^{-3}}
\@namedef{num@mv2.curvedtent.10000.mse}{2.1\times10^{-13}}
\@namedef{num@mv2.curvedtent.10000.un}{2.4\times10^{-3}}
\@namedef{num@mv2.mse.fmax}{3\times10^{6}}
\@namedef{num@mv2.mse.fmin}{4.3}
\@namedef{num@mv2.mse.within}{0}
\@namedef{num@mv2.quadtent.1000.mse}{3.5\times10^{-11}}
\@namedef{num@mv2.quadtent.1000.un}{3.2\times10^{-3}}
\@namedef{num@mv2.quadtent.10000.mse}{3.6\times10^{-12}}
\@namedef{num@mv2.quadtent.10000.un}{4.1\times10^{-3}}
\@namedef{num@mv2.un.within}{5}
\@namedef{num@noise.2.cs.clean}{5.1\times10^{-16}}
\@namedef{num@noise.2.exact.max}{2.7}
\@namedef{num@noise.2.exact.min}{2.4}
\@namedef{num@noise.2.m}{5}
\@namedef{num@noise.2.zero.clean}{76}
\@namedef{num@noise.2.zero.max}{21}
\@namedef{num@noise.4.cs.clean}{1.4\times10^{-14}}
\@namedef{num@noise.4.lc}{3.0\times10^{-15}}
\@namedef{num@noise.4.zero.clean}{39}
\@namedef{num@noise.4.zero.max}{11}
\@namedef{num@noise.5.cs.clean}{4.1\times10^{-15}}
\@namedef{num@noise.5.zero.clean}{32}
\@namedef{num@noise.5.zero.max}{9}
\@namedef{num@noise.6.cs.clean}{5.8\times10^{-15}}
\@namedef{num@noise.6.zero.clean}{26}
\@namedef{num@noise.6.zero.max}{7}
\@namedef{num@noise.cells}{20}
\@namedef{num@noise.cs.best}{12}
\@namedef{num@noise.decades}{8}
\@namedef{num@noise.hi.ratio.max}{1.13}
\@namedef{num@noise.hi.ratio.min}{0.95}
\@namedef{num@noise.kink.exact.max}{1.7}
\@namedef{num@noise.kink.exact.min}{1.2}
\@namedef{num@noise.kink.m.clean}{1}
\@namedef{num@noise.kink.m.max}{3}
\@namedef{num@noise.kink.m.min}{2}
\@namedef{num@noise.low.max}{540}
\@namedef{num@noise.low.min}{386}
\@namedef{num@noise.ratio.max}{1.13}
\@namedef{num@noise.ratio.min}{0.68}
\@namedef{num@noise.refit.off}{4}
\@namedef{num@noise.splats.clean.max}{605}
\@namedef{num@noise.splats.clean.min}{339}
\@namedef{num@noise.splats.hi.max}{188}
\@namedef{num@noise.splats.hi.min}{108}
\@namedef{num@noise.zero.maxgap}{one step}
\@namedef{num@pp.10000.best}{13.64}
\@namedef{num@pp.10000.deg}{7}
\@namedef{num@pp.10000.sel}{13.26}
\@namedef{num@pp.10000.sel64}{13.26}
\@namedef{num@pp.2000.best}{13.66}
\@namedef{num@pp.2000.deg}{6}
\@namedef{num@pp.2000.sel}{13.51}
\@namedef{num@pp.2000.sel64}{13.51}
\@namedef{num@pp.400.best}{11.85}
\@namedef{num@pp.400.deg}{6}
\@namedef{num@pp.400.sel}{11.85}
\@namedef{num@pp.400.sel64}{11.85}
\@namedef{num@pp.best.max}{13.66}
\@namedef{num@pp.digits.min}{111}
\@namedef{num@pp.map.deg}{128}
\@namedef{num@pp.map.dev}{10^{-7}}
\@namedef{num@pp.map.digits.min}{52}
\@namedef{num@pp.map.ratio.max}{2\times10^{8}}
\@namedef{num@pp.map.ratio.min}{2\times10^{7}}
\@namedef{num@pp.qmax}{15}
\@namedef{num@pyedm.4.n}{49{,}998}
\@namedef{num@pyedm.4.ours}{1.609\times10^{-15}}
\@namedef{num@pyedm.4.pyedm}{1.611\times10^{-15}}
\@namedef{num@rbf.cells}{9}
\@namedef{num@rbf.mse.phrase}{all 9}
\@namedef{num@rbf.mse.wins}{9}
\@namedef{num@rbf.numbers.max}{8{,}005}
\@namedef{num@rbf.numbers.min}{4{,}003}
\@namedef{num@rbf.ratio.max}{3\times10^{7}}
\@namedef{num@rbf.ratio.min}{120}
\@namedef{num@rbf.un.phrase}{all 9}
\@namedef{num@rbf.un.wins}{9}
\@namedef{num@ros.ar.mse}{2.2\times10^{-10}}
\@namedef{num@ros.ar.un}{4.1\times10^{-3}}
\@namedef{num@ros.best.mse}{2.5\times10^{-14}}
\@namedef{num@ros.best.name}{Local polynomial, own window}
\@namedef{num@ros.best20.name}{Local polynomial, own window}
\@namedef{num@ros.best20.un}{5.6\times10^{-15}}
\@namedef{num@ros.cs.m}{12}
\@namedef{num@ros.cs.mse}{3.7\times10^{-14}}
\@namedef{num@ros.cs.size}{2.0\times10^{4}}
\@namedef{num@ros.cs.splats}{185}
\@namedef{num@ros.cs.un}{2.7\times10^{-12}}
\@namedef{num@ros.esn.m}{100}
\@namedef{num@ros.esn.mse}{1.8\times10^{-7}}
\@namedef{num@ros.esn.un}{1.4\times10^{-5}}
\@namedef{num@ros.lp.m}{12}
\@namedef{num@ros.lp.mse}{2.7\times10^{-14}}
\@namedef{num@ros.lp.un}{1.6\times10^{-14}}
\@namedef{num@ros.lpo.m}{16}
\@namedef{num@ros.lpo.mse}{2.5\times10^{-14}}
\@namedef{num@ros.lpo.un}{5.6\times10^{-15}}
\@namedef{num@ros.ngrc.m}{16}
\@namedef{num@ros.ngrc.mse}{1.1\times10^{-13}}
\@namedef{num@ros.ngrc.un}{4.6\times10^{-1}}
\@namedef{num@ros.poly.m}{8}
\@namedef{num@ros.poly.mse}{1.4\times10^{-13}}
\@namedef{num@ros.poly.un}{4.3\times10^{-10}}
\@namedef{num@ros.ratio}{0.66}
\@namedef{num@ros.ratio20}{0.0021}
\@namedef{num@ros.ratioglobal}{3}
\@namedef{num@ros.rbf.m}{12}
\@namedef{num@ros.rbf.mse}{2.7\times10^{-13}}
\@namedef{num@ros.rbf.un}{1.3\times10^{-10}}
\@namedef{num@ros.smap.m}{12}
\@namedef{num@ros.smap.mse}{5.9\times10^{-14}}
\@namedef{num@ros.smap.un}{2.9\times10^{-12}}
\@namedef{num@ros.smapo.m}{9}
\@namedef{num@ros.smapo.mse}{6.5\times10^{-14}}
\@namedef{num@ros.smapo.un}{4.0\times10^{-12}}
\@namedef{num@s1b.bands}{18}
\@namedef{num@s1b.forecasts}{4\times10^{6}}
\@namedef{num@s1b.inband}{171}
\@namedef{num@s1b.outside}{6}
\@namedef{num@s1b.splats}{171}
\@namedef{num@s1b.width}{0.0086}
\@namedef{num@s1b.windows}{200}
\@namedef{num@s1b.worst}{6\times10^{-8}}
\@namedef{num@sf.ESN.100}{39.}
\@namedef{num@sf.ESN.25}{0.00043}
\@namedef{num@sf.ESN.50}{0.037}
\@namedef{num@sf.ESNtuned.100}{$1.4\times10^{8}$}
\@namedef{num@sf.ESNtuned.25}{0.00031}
\@namedef{num@sf.ESNtuned.50}{0.0017}
\@namedef{num@sf.FarmerSidorowichlocalpolynomial.100}{1.0}
\@namedef{num@sf.FarmerSidorowichlocalpolynomial.25}{0.0060}
\@namedef{num@sf.FarmerSidorowichlocalpolynomial.50}{0.39}
\@namedef{num@sf.FarmerSidorowichlocalpolynomialgridv1.100}{1.0}
\@namedef{num@sf.FarmerSidorowichlocalpolynomialgridv1.25}{0.0060}
\@namedef{num@sf.FarmerSidorowichlocalpolynomialgridv1.50}{0.39}
\@namedef{num@sf.GSCN.100}{0.70}
\@namedef{num@sf.GSCN.25}{0.0010}
\@namedef{num@sf.GSCN.50}{0.051}
\@namedef{num@sf.LSTM.100}{0.92}
\@namedef{num@sf.LSTM.25}{0.0076}
\@namedef{num@sf.LSTM.50}{0.15}
\@namedef{num@sf.NGRCtuned.100}{diverged}
\@namedef{num@sf.NGRCtuned.25}{diverged}
\@namedef{num@sf.NGRCtuned.50}{diverged}
\@namedef{num@sf.SmapSugihara.100}{0.68}
\@namedef{num@sf.SmapSugihara.25}{0.0030}
\@namedef{num@sf.SmapSugihara.50}{0.0082}
\@namedef{num@sf.SmapSugiharagridv1.100}{0.74}
\@namedef{num@sf.SmapSugiharagridv1.25}{0.0029}
\@namedef{num@sf.SmapSugiharagridv1.50}{0.0084}
\@namedef{num@sf.cs.m}{10}
\@namedef{num@sf.globalpolynomialNGRCstyle.100}{diverged}
\@namedef{num@sf.globalpolynomialNGRCstyle.25}{0.0013}
\@namedef{num@sf.globalpolynomialNGRCstyle.50}{0.20}
\@namedef{num@size.bytes.mse.wins}{6}
\@namedef{num@size.bytes.un.wins}{6}
\@namedef{num@size.cells}{9}
\@namedef{num@size.first.cells}{9}
\@namedef{num@size.first.mse.wins}{9}
\@namedef{num@size.first.phrase}{all 9}
\@namedef{num@size.loss.max}{370}
\@namedef{num@size.loss.min}{33}
\@namedef{num@size.loss.where}{the border-collision map ($10^{5}$ and $9\times10^{5}$ points) and the Lozi map ($10^{5}$ points)}
\@namedef{num@size.loss.who}{the S-map on error-selected points}
\@namedef{num@size.mse.max}{5\times10^{3}}
\@namedef{num@size.mse.min}{1.7}
\@namedef{num@size.mse.wins}{6}
\@namedef{num@size.numbers.max}{17{,}001}
\@namedef{num@size.numbers.min}{1{,}690}
\@namedef{num@size.small.cells}{6}
\@namedef{num@size.small.mse.losses}{4}
\@namedef{num@size.smooth.max}{1.2}
\@namedef{num@size.un.max}{3.6}
\@namedef{num@size.un.wins}{7}
\@namedef{num@smooth.globalfloor.max}{8.5}
\@namedef{num@smooth.ratiofloor.max}{2.5}
\@namedef{num@smooth.rbffloor.max}{3.8}
\@namedef{num@train.cs.max}{69}
\@namedef{num@train.cs.min}{51}
\@namedef{num@train.local.max}{2.8}
\@namedef{num@train.local.min}{0.26}
\@namedef{num@vb.1.best}{1.00}
\@namedef{num@vb.1.bestend}{20}
\@namedef{num@vb.1.cs}{1.00}
\@namedef{num@vb.1.exact}{1.00}
\@namedef{num@vb.2.best}{0.88}
\@namedef{num@vb.2.bestend}{20}
\@namedef{num@vb.2.cs}{1.00}
\@namedef{num@vb.2.exact}{1.00}
\@namedef{num@vb.3.best}{0.63}
\@namedef{num@vb.3.bestend}{20}
\@namedef{num@vb.3.cs}{1.00}
\@namedef{num@vb.3.exact}{0.98}
\@namedef{num@vb.4.best}{0.18}
\@namedef{num@vb.4.bestend}{20}
\@namedef{num@vb.4.cs}{0.83}
\@namedef{num@vb.4.exact}{0.73}
\@namedef{num@vb.5.best}{-0.04}
\@namedef{num@vb.5.bestend}{17}
\@namedef{num@vb.5.cs}{0.47}
\@namedef{num@vb.5.exact}{0.41}
\@namedef{num@vb.6.best}{0.19}
\@namedef{num@vb.6.bestend}{20}
\@namedef{num@vb.6.cs}{0.18}
\@namedef{num@vb.6.exact}{0.18}
\@namedef{num@vb.ratio.max}{5\times10^{9}}
\@namedef{num@vb.ratio.min}{6\times10^{7}}
\@namedef{num@vbad.1.max}{14}
\@namedef{num@vbad.1.min}{1.7}
\@namedef{num@win.2.cs}{75.1}
\@namedef{num@win.2.equal}{67}
\@namedef{num@win.2.gap}{0.1}
\@namedef{num@win.2.gap.hi}{0.9}
\@namedef{num@win.2.gap.lo}{-0.6}
\@namedef{num@win.2.longer}{17}
\@namedef{num@win.2.name}{the global polynomial}
\@namedef{num@win.2.other}{75.2}
\@namedef{num@win.2.shorter}{16}
\@namedef{num@win.3.cs}{51.0}
\@namedef{num@win.3.equal}{84}
\@namedef{num@win.3.gap}{0.3}
\@namedef{num@win.3.gap.hi}{0.7}
\@namedef{num@win.3.gap.lo}{-0.1}
\@namedef{num@win.3.longer}{7}
\@namedef{num@win.3.name}{the Farmer--Sidorowich predictor}
\@namedef{num@win.3.other}{51.4}
\@namedef{num@win.3.shorter}{9}
\@namedef{num@win.4.cs}{40.7}
\@namedef{num@win.4.equal}{35}
\@namedef{num@win.4.gap}{0.0}
\@namedef{num@win.4.gap.hi}{0.5}
\@namedef{num@win.4.gap.lo}{-0.5}
\@namedef{num@win.4.longer}{34}
\@namedef{num@win.4.name}{the Farmer--Sidorowich predictor}
\@namedef{num@win.4.other}{40.7}
\@namedef{num@win.4.shorter}{31}
\@namedef{num@win.5.cs}{32.1}
\@namedef{num@win.5.equal}{50}
\@namedef{num@win.5.gap}{0.1}
\@namedef{num@win.5.gap.hi}{0.5}
\@namedef{num@win.5.gap.lo}{-0.3}
\@namedef{num@win.5.longer}{25}
\@namedef{num@win.5.name}{the Farmer--Sidorowich predictor}
\@namedef{num@win.5.other}{32.3}
\@namedef{num@win.5.shorter}{25}
\@namedef{num@win.6.cs}{26.1}
\@namedef{num@win.6.equal}{46}
\@namedef{num@win.6.gap}{0.1}
\@namedef{num@win.6.gap.hi}{0.3}
\@namedef{num@win.6.gap.lo}{-0.5}
\@namedef{num@win.6.longer}{28}
\@namedef{num@win.6.name}{the S-map}
\@namedef{num@win.6.other}{26.0}
\@namedef{num@win.6.shorter}{25}
\@namedef{num@win.cells}{6}
\@namedef{num@win.check.max}{3\times10^{-8}}
\@namedef{num@win.equal.max}{84}
\@namedef{num@win.equal.min}{35}
\@namedef{num@win.henon.cs}{86.7}
\@namedef{num@win.henon.equal}{46}
\@namedef{num@win.henon.gap}{1.7}
\@namedef{num@win.henon.gap.hi}{2.6}
\@namedef{num@win.henon.gap.lo}{0.8}
\@namedef{num@win.henon.longer}{19}
\@namedef{num@win.henon.name}{the Farmer--Sidorowich predictor on its own window}
\@namedef{num@win.henon.other}{88.4}
\@namedef{num@win.henon.shorter}{36}
\@namedef{num@win.same.count}{5}
\@namedef{num@win.same.halfwidth}{0.9}
\@namedef{num@win.windows.min}{2{,}993}
\makeatother


==> tables/rollout_numbers.tex <==
% generated by experiments/paper_figures/fig_fresh_rollouts.py -- do not edit
\makeatletter
\@namedef{num@roll.full.exact.max}{1.06}
\@namedef{num@roll.full.exact.median}{1.00}
\@namedef{num@roll.full.exact.min}{0.98}
\@namedef{num@roll.full.lead.max}{7}
\@namedef{num@roll.full.lead.min}{1}
\@namedef{num@roll.full.longest}{18}
\@namedef{num@roll.full.medratio}{1.04}
\@namedef{num@roll.full.strict}{18}
\@namedef{num@roll.full.units}{18}
\@namedef{num@roll.ross.cap}{25{,}000}
\@namedef{num@roll.ross.esn.A}{0.84}
\@namedef{num@roll.ross.esn.B}{0.90}
\@namedef{num@roll.ross.esn.steps.A}{6{,}000}
\@namedef{num@roll.ross.esn.steps.B}{6{,}000}
\@namedef{num@roll.ross.esn.unexpl.atesn.A}{0.16}
\@namedef{num@roll.ross.esn.unexpl.atesn.B}{0.10}
\@namedef{num@roll.ross.esn.unexpl.atlp.A}{7.3\times10^{-5}}
\@namedef{num@roll.ross.esn.unexpl.atlp.B}{8.4\times10^{-8}}
\@namedef{num@roll.ross.lp.A}{1.00}
\@namedef{num@roll.ross.lp.B}{1.00}
\@namedef{num@roll.ross.lp.steps.A}{1{,}383}
\@namedef{num@roll.ross.lp.steps.B}{1{,}399}
\@namedef{num@roll.ross.lp.unexpl.atlp.A}{3.9\times10^{-9}}
\@namedef{num@roll.ross.lp.unexpl.atlp.B}{9.4\times10^{-10}}
\@namedef{num@roll.ross.smap.A}{0.42}
\@namedef{num@roll.ross.smap.B}{0.57}
\@namedef{num@roll.ross.smap.steps.A}{25{,}000}
\@namedef{num@roll.ross.smap.steps.B}{25{,}000}
\@namedef{num@roll.ross.smap.unexpl.atesn.A}{0.23}
\@namedef{num@roll.ross.smap.unexpl.atesn.B}{0.19}
\@namedef{num@roll.ross.smap.unexpl.atlp.A}{1.0\times10^{-2}}
\@namedef{num@roll.ross.smap.unexpl.atlp.B}{1.3\times10^{-3}}
\@namedef{num@roll.ross.v4.A}{0.71}
\@namedef{num@roll.ross.v4.B}{0.66}
\@namedef{num@roll.ross.v4.steps.A}{25{,}000}
\@namedef{num@roll.ross.v4.steps.B}{25{,}000}
\@namedef{num@roll.ross.v4.unexpl.atesn.A}{0.06}
\@namedef{num@roll.ross.v4.unexpl.atesn.B}{0.06}
\@namedef{num@roll.ross.v4.unexpl.atlp.A}{3.7\times10^{-10}}
\@namedef{num@roll.ross.v4.unexpl.atlp.B}{6.4\times10^{-10}}
\makeatother


==> tables/supp_labels_arxiv.tex <==
% generated by make_journal.py from gscn_supplement.aux (tables the arXiv version omits) -- do not edit
\makeatletter
\@namedef{supp@sec:networks-full}{S1}
\@namedef{supp@eq:coherence}{1}
\@namedef{supp@eq:stretch}{3}
\@namedef{supp@sec:safeguards}{S2}
\@namedef{supp@eq:guard}{5}
\@namedef{supp@sec:closedloop}{S3}
\@namedef{supp@eq:valhorizon}{6}
\@namedef{supp@sec:polyrelation}{S4}
\@namedef{supp@tab:polymodels}{S1}
\@namedef{supp@sec:stencil-method}{S5}
\@namedef{supp@sec:cost-full}{S6}
\@namedef{supp@sec:v4-longcost}{S7}
\@namedef{supp@eq:views}{7}
\@namedef{supp@sec:baselines-full}{S8}
\@namedef{supp@tab:regimes}{S2}
\@namedef{supp@tab:cost}{S3}
\@namedef{supp@fig:budget}{S1}
\@namedef{supp@fig:budget-cost}{S2}
\@namedef{supp@tab:budget-cost}{S4}
\@namedef{supp@tab:budget-targets}{S5}
\@namedef{supp@tab:budget-small}{S6}
\@namedef{supp@sec:henon}{S17}
\@namedef{supp@sec:flows}{S18}
\@namedef{supp@tab:flows}{S7}
\@namedef{supp@fig:santafe}{S3}
\@namedef{supp@tab:santafe}{S8}
\@namedef{supp@sec:dysts}{S23}
\@namedef{supp@fig:dysts}{S4}
\@namedef{supp@sec:longr2}{S24}
\@namedef{supp@tab:longr2}{S9}
\@namedef{supp@fig:long-smooth}{S5}
\@namedef{supp@fig:long-kinked}{S6}
\@namedef{supp@fig:noise}{S7}
\@namedef{supp@tab:noise-full}{S10}
\@namedef{supp@tab:abl-dims}{S11}
\@namedef{supp@sec:noise-full}{S30}
\@namedef{supp@sec:l63}{S32}
\@namedef{supp@tab:l63}{S12}
\@namedef{supp@sec:l96}{S33}
\@namedef{supp@sec:smooth-full}{S34}
\@namedef{supp@tab:fresh910}{S13}
\@namedef{supp@tab:fresh11}{S14}
\@namedef{supp@tab:v4-robust}{S15}
\@namedef{supp@tab:fresh-rollouts}{S16}
\@namedef{supp@tab:ladder910}{S17}
\@namedef{supp@tab:pointdist910}{S18}
\@namedef{supp@sec:fresh-full}{S42}
\@namedef{supp@sec:fairness-more}{S43}
\@namedef{supp@tab:cheat}{S19}
\@namedef{supp@tab:criticisms}{S20}
\@namedef{supp@sec:fairness-full}{S46}
\@namedef{supp@sec:hidden}{S48}
\@namedef{supp@sec:extra-baselines}{S52}
\@namedef{supp@tab:extra-baselines}{S21}
\@namedef{supp@sec:polyprop-fresh}{S53}
\@namedef{supp@tab:polyprop}{S22}
\@namedef{supp@fig:kink-errors}{S8}
\@namedef{supp@sec:machine}{S55}
\@namedef{supp@tab:datasets}{S23}
\@namedef{supp@tab:baselines}{S24}
\@namedef{supp@tab:complexity}{S25}
\@namedef{supp@tab:heldout2}{S26}
\@namedef{supp@tab:abl-components}{S27}
\@namedef{supp@tab:learning}{S28}
\@namedef{supp@app:tables}{S57}
\@namedef{supp@tab:maps-baselines}{S29}
\@namedef{supp@tab:l96}{S30}
\@namedef{supp@app:v4spec}{S58}
\makeatother


==> tables/system_numbers.tex <==
% written by make_system_numbers.py from v4_units.json
\makeatletter\@namedef{num@sys.n}{10}\makeatother
\makeatletter\@namedef{num@sys.allresolved}{10}\makeatother
\makeatletter\@namedef{num@sys.inv.median}{121}\makeatother
\makeatletter\@namedef{num@sys.inv.min}{1.75}\makeatother
\makeatletter\@namedef{num@sys.inv.max}{1.8\times10^{7}}\makeatother
\makeatletter\@namedef{num@sys.inv.min.name}{R\"ossler}\makeatother


==> tables/traj_numbers.tex <==
% generated by paper_figures/fig_lozi_trajectory.py -- do not edit
\makeatletter
\@namedef{num@traj.windows}{200}
\@namedef{num@traj.steps}{60}
\@namedef{num@traj.v4.valid}{34}
\@namedef{num@traj.v4.mae5}{1.7\times10^{-7}}
\@namedef{num@traj.v4.mae10}{2.1\times10^{-6}}
\@namedef{num@traj.v4.mae20}{2.9\times10^{-4}}
\@namedef{num@traj.smap.valid}{33}
\@namedef{num@traj.smap.mae5}{1.3\times10^{-4}}
\@namedef{num@traj.smap.mae10}{1.1\times10^{-3}}
\@namedef{num@traj.smap.mae20}{2.6\times10^{-2}}
\@namedef{num@traj.lp.valid}{32}
\@namedef{num@traj.lp.mae5}{8.0\times10^{-5}}
\@namedef{num@traj.lp.mae10}{8.2\times10^{-4}}
\@namedef{num@traj.lp.mae20}{1.8\times10^{-2}}
\@namedef{num@traj.exact.valid}{34}
\@namedef{num@traj.exact.mae5}{2.2\times10^{-7}}
\@namedef{num@traj.exact.mae10}{2.6\times10^{-6}}
\@namedef{num@traj.exact.mae20}{3.8\times10^{-4}}
\@namedef{num@traj.smap.step1max}{1.3\times10^{-3}}
\@namedef{num@traj.v4.step1max}{1.2\times10^{-7}}
\@namedef{num@traj.longer}{123}
\@namedef{num@traj.shorter}{50}
\@namedef{num@traj.longer5}{43}
\@namedef{num@traj.shorter5}{8}
\@namedef{num@traj.v4.onestep}{9.0\times10^{-16}}
\makeatother


==> tables/v4_numbers.tex <==
% generated by experiments/overleaf/make_v4_tables.py from the confirmation results -- do not edit
\makeatletter
\@namedef{num@f11.dominated.base}{15}
\@namedef{num@f11.dominated.cs}{1}
\@namedef{num@f11.median.units}{19}
\@namedef{num@f11.median.wins}{19}
\@namedef{num@f11.oneseed.units}{19}
\@namedef{num@f11.oneseed.wins}{19}
\@namedef{num@f11.ratio.medianinv}{1197}
\@namedef{num@f11.resolved}{19}
\@namedef{num@f11.roll.units}{19}
\@namedef{num@f11.roll20.wins}{19}
\@namedef{num@f11.roll5.wins}{18}
\@namedef{num@f11.sys}{19}
\@namedef{num@f11.syswins}{19}
\@namedef{num@f11.units}{19}
\@namedef{num@f11.unitwins}{19}
\@namedef{num@f78.oneseed.units}{38}
\@namedef{num@f78.oneseed.wins}{36}
\@namedef{num@f78.resolved}{36}
\@namedef{num@f78.roll.units}{38}
\@namedef{num@f78.roll20.wins}{37}
\@namedef{num@f78.roll5.wins}{37}
\@namedef{num@f78.sys}{19}
\@namedef{num@f78.syswins}{17}
\@namedef{num@f78.units}{38}
\@namedef{num@f78.unitwins}{36}
\@namedef{num@f78.v1.units}{38}
\@namedef{num@f78.v1.wins}{11}
\@namedef{num@f78.v2.units}{36}
\@namedef{num@f78.v2.wins}{34}
\@namedef{num@f78.v3.units}{38}
\@namedef{num@f78.v3.wins}{36}
\@namedef{num@f910.dominated.base}{27}
\@namedef{num@f910.dominated.cs}{1}
\@namedef{num@f910.final.units}{38}
\@namedef{num@f910.final.wins}{38}
\@namedef{num@f910.median.units}{38}
\@namedef{num@f910.median.wins}{38}
\@namedef{num@f910.netalone.units}{32}
\@namedef{num@f910.netalone.wins}{29}
\@namedef{num@f910.oneseed.units}{38}
\@namedef{num@f910.oneseed.wins}{36}
\@namedef{num@f910.own.better}{222}
\@namedef{num@f910.own.points}{232}
\@namedef{num@f910.own.queries}{1\,598\,944}
\@namedef{num@f910.par.serial}{0.6}
\@namedef{num@f910.par.speedup.1e4}{2.7}
\@namedef{num@f910.par.speedup.1e5}{2.8}
\@namedef{num@f910.pred.1e4.base}{12}
\@namedef{num@f910.pred.1e4.cs}{287}
\@namedef{num@f910.pred.1e5.base}{13}
\@namedef{num@f910.pred.1e5.cs}{441}
\@namedef{num@f910.pred.ratio}{24}
\@namedef{num@f910.ratio.max}{0.814}
\@namedef{num@f910.ratio.median}{0.014}
\@namedef{num@f910.ratio.medianinv}{72}
\@namedef{num@f910.ratio.min}{8.5\times10^{-9}}
\@namedef{num@f910.ref.asked}{61}
\@namedef{num@f910.ref.changed}{3.9}
\@namedef{num@f910.resolved}{38}
\@namedef{num@f910.roll.units}{38}
\@namedef{num@f910.roll20.wins}{38}
\@namedef{num@f910.roll5.wins}{38}
\@namedef{num@f910.scale.coef}{0.18}
\@namedef{num@f910.scale.fit}{0.91}
\@namedef{num@f910.scale.fit.max}{1.23}
\@namedef{num@f910.scale.fit.min}{0.79}
\@namedef{num@f910.scale.lpfit}{0.53}
\@namedef{num@f910.scale.pairs}{18}
\@namedef{num@f910.scale.pred}{0.07}
\@namedef{num@f910.scale.smfit}{0.81}
\@namedef{num@f910.sys}{19}
\@namedef{num@f910.syswins}{19}
\@namedef{num@f910.time.1e4.base}{33}
\@namedef{num@f910.time.1e4.cs}{24}
\@namedef{num@f910.time.1e4.own}{12}
\@namedef{num@f910.time.1e5.base}{2.4}
\@namedef{num@f910.time.1e5.cs}{3.1}
\@namedef{num@f910.time.1e5.own}{2}
\@namedef{num@f910.timedout}{0}
\@namedef{num@f910.units}{38}
\@namedef{num@f910.unitwins}{38}
\@namedef{num@f910.v1.units}{37}
\@namedef{num@f910.v1.wins}{15}
\@namedef{num@f910.v2.units}{35}
\@namedef{num@f910.v2.wins}{34}
\@namedef{num@f910.v3.units}{38}
\@namedef{num@f910.v3.wins}{37}
\@namedef{num@f910.vsfinal.better}{13}
\@namedef{num@f910.vsfinal.big}{5}
\@namedef{num@f910.vsfinal.geo}{0.51}
\@namedef{num@f910.vsfinal.maxgain}{3.6\times10^{3}}
\@namedef{num@f910.vsfinal.maxloss}{1.42}
\@namedef{num@f910.vsfinal.mingain}{5.52}
\@namedef{num@f910.vsfinal.units}{32}
\@namedef{num@f910.vsfinal.worse}{19}
\@namedef{num@f911.resolved}{57}
\@namedef{num@f911.units}{57}
\@namedef{num@f911.unitwins}{57}
\@namedef{num@ppf.degree.max}{223}
\@namedef{num@ppf.div20}{29}
\@namedef{num@ppf.kink.max}{2.7\times10^{11}}
\@namedef{num@ppf.kink.min}{6.1\times10^{5}}
\@namedef{num@ppf.loss.pct}{2}
\@namedef{num@ppf.loss.unit}{Series 3, $n=10^{4}$, initial condition A}
\@namedef{num@ppf.losses}{1}
\@namedef{num@ppf.resolved}{37}
\@namedef{num@ppf.units}{38}
\@namedef{num@ppf.wins}{37}
\makeatother

